Data Augmentation for Deep Receivers

Deep neural networks (DNNs) allow digital receivers to learn to operate in complex environments. To do so, DNNs should preferably be trained using large labeled data sets with a similar statistical relationship as the one under which they are to infer. For DNN-aided receivers, obtaining labeled data conventionally involves pilot signalling at the cost of reduced spectral efficiency, typically resulting in access to limited data sets. In this paper, we study how one can enrich a small set of labeled pilots data into a larger data set for training deep receivers. Motivated by the widespread use of data augmentation techniques for enriching visual and text data, we propose dedicated augmentation schemes that exploits the characteristics of digital communication data. We identify the key considerations in data augmentations for deep receivers as the need for domain orientation, class (constellation) diversity, and low complexity. Following these guidelines, we devise three complementing augmentations that exploit the geometric properties of digital constellations. Our combined augmentation approach builds on the merits of these different augmentations to synthesize reliable data from a momentary channel distribution, to be used for training deep receivers. Furthermore, we exploit previous channel realizations to increase the reliability of the augmented samples.

==> sections/abstract.tex <==
\begin{abstract} 
\TomerFill{Deep neural networks (DNNs) allow digital receivers to learn to operate in complex environments. To do so, DNNs should  preferably be trained using large labeled data sets with a similar statistical relationship as the one under which they are to infer. For DNN-aided receivers, obtaining labeled data  conventionally involves pilot signalling at the cost of reduced spectral efficiency, typically resulting in access to limited data sets.
In this paper, we study how one can enrich a small set of labeled data into a larger data set for training deep receivers without transmitting more pilots. Motivated by the widespread use of data augmentation techniques for enriching visual and text data, we propose a dedicated augmentation scheme for exploiting the characteristics of digital communication data.  We identify the key considerations in data augmentations  for deep receivers as the need for domain orientation, class (constellation) diversity, and low complexity. Our method models each symbols class as Gaussian, using the available data to estimate its moments, while possibly leveraging data corresponding to related statistical models, e.g., past channel realizations, to improve the estimate.
The estimated clusters are used to enrich the data set by generating new samples used for training the DNN. The superiority of our approach is numerically evaluated for training a deep receiver on a linear and non-linear synthetic channels, as well as a COST 2100 channel. We show that our augmentation allows DNN-aided receivers to achieve gain of up to 3dB in \acl{ber}, compared to regular non-augmented training.} Should replace later.
\end{abstract}

==> sections/conclusion.tex <==
\section{Conclusion}
	\label{sec:conclusion}
	\vspace{-0.1cm}
In this paper, we have proposed ...

==> sections/dynamic.tex <==
% TODO NIR CONTINUE FROM HERE

\section{Data Augmentations for Dynamic Channels}
\label{sec:data_augmentations_dynamic}

\textcolor{red}{can you please add an illustration for this approach? we had something of that sort in your slides}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/adaptive augmentation.PNG}
    \caption{Time-varying channels may benefit from an adaptive augmentation scheme. \textcolor{red}{please make the 'Block Index j' text smaller, and add the mathematical notations on top of the figure}}
    \label{fig:adaptive_augmentation_illustration}
\end{figure}

In practice, digital receivers often operate in block-fading channel conditions. In such cases,  each block of $B$ symbols undergoes a different channel, i.e., the statistical relationship between the channel outputs at the $j$th block $\{\myVec{y}_{i,j}\}_{i=1}^{\Blklen}$ and the  symbols $\{\myVec{s}_{i,j}\}_{i=1}^{\Blklen}$ varies with $j$. While each block requires a different receiver mapping $\Weights_j$, the data augmentation scheme $\psi$ can possibly fine tune itself between different realizations. For such settings, we are interested in data augmentation schemes that are {\em adaptive}, and are capable of leveraging past channel realizations to improve their ability to synthesize useful training data $\mySet{Q}^*$ from the current pilots\textcolor{blue}{, as illustrated in Fig.~\ref{fig:adaptive_augmentation_illustration}}. Since in this section the proposed scheme is adaptive, the mapping $\psi$ depends not only on the available data $\mySet{Q}$, but also on the previously used augmentation, i.e., the mapping applied in the previous block for block fading settings, denoted $\psi_{\rm prev}$. 

In block-fading settings, we propose to adaptively smooth the estimated clusters parameters \eqref{eq:mean_calculation} and \eqref{eq:variance_calculation} via a window smoothing approach. This way, we combine data across multiple time frames, meanwhile reducing the estimation noise. The motivation stems from the fact that  adjacent blocks may have different number of samples per class in each block, which induces high-variance noise. To reduce the noise effects, we exploit the continuous operation of \ac{dnn}-aided receivers and incorporate  adaptive smoothing, updating the clustering via
\begin{equation} \label{eq:smoothed_mean_calculation}
    \myVec{\mu}(\mypoint) = \frac{\alpha_1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \myVec{y}_{i} + (1-\alpha_1) * \myVec{\mu}_{\rm prev}(\mypoint) ,
\end{equation}
and
\begin{equation} \label{eq:smoothed_variance_calculation}
    \!\!\myMat{\Sigma}(\mypoint) \!=\!\frac{\alpha_2}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \!\!\!\!(\myVec{y}_{i}\! - \!\myVec{\mu}(\mypoint))(\myVec{y}_{i} \!-\! \myVec{\mu}(\mypoint))^T + (1-\alpha_2) * \myMat{\Sigma}_{\rm prev}(\mypoint).
\end{equation}
Here,  $\alpha_1,\alpha_2 \in [0,1]$ are hyperparameters  balancing the contribution of $\psi_{\rm prev}$ on $\psi$. For $\alpha_1=\alpha_2=1$, $\psi$ is not adaptive and is determined solely by $\mySet{Q}$, while for $\alpha_1=\alpha_2 = 0$, we have $\psi \equiv \psi_{\rm prev}$. 

To conclude the dynamic channel augmentation scheme $\psi_{dynamic}$, we follow the same guidelines of Algorithm~\ref{alg:StaticAugmentationScheme}, while replacing only lines \ref{line:centers_calculation} and \ref{line:variance_calculation} with the calculations in equations \eqref{eq:smoothed_mean_calculation} and \eqref{eq:smoothed_variance_calculation}, respectively.

==> sections/introduction.tex <==
\section{Introduction}
\vspace{-0.1cm} 
	
% Paragraph - deep learning for receivers
% An alternative data-driven approach is based on deep learning. 
The emergence of deep learning has notably impacted numerous applications in various disciplines. %, ranging from computer vision and natural language processing to speech refinement and biomedical signal processing. 
The ability of \acp{dnn} to learn to efficiently carry out complex tasks from data has spurred a growing interest in their usage for receiver design in digital communications \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, farsad2020data}. The integration of model-agnostic trainable \acp{dnn}  in the receiver processing facilitates operation in complex scenarios where either a channel model deficit or an efficient algorithm deficit exist \cite{oshea2017introduction}, and can thus greatly contribute to meeting the constantly growing requirements of wireless systems in terms of throughput, coverage, and robustness \cite{saad2019vision}. 

% Following the same path, researchers in digital communication started to implement \ac{ml} driven solutions in classic communication components, such as antennas \cite{shlezinger2020dynamic}, reconfigurable intelligent surfaces \cite{alexandropoulos2021hybrid} and receivers \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, oshea2017introduction}. While traditional receiver algorithms are channel-model-based, relying on mathematical modeling \cite{xia2020mimo} of the signal transmission, propagation, and reception, \ac{dnn}-based receivers may facilitate operation in complex scenarios where either a channel model deficit or an efficient algorithm deficit exist \cite{shlezinger2020dynamic,alexandropoulos2021hybrid}, or difficult to optimize for~\cite{farsad2018neural,shlezinger2018asymptotic}.

% Paragraph - inherent challenge due to small available data sets
While deep learning thrives in domains such as computer vision or natural language processing, many challenges still limit its widespread applicability in digital communications. One of these challenges arises from the fact that \acp{dnn} rely on  (typically labeled) data sets to learn their mappings, and are thus usually applied when the  function being learned is stationary for a long period of time, such that one can collect sufficient data for learning. For example, data sets for machine translation tasks, which are nowadays dominated by deep learning systems, are usually composed of a sentence in an origin language, and its respective translation in a destination language, which does not change in time. One can thus collect millions or billions of such pairs for training, obtaining a huge data set for the task at hand. 
%
In contrast, the operation of digital receivers is rarely stationary, as communication channels (and thus the distribution of the data) change considerably over time. Moreover, \acp{dnn} are  highly-parameterized models, and their training requires massive data sets. In  digital receivers, labeled data corresponding to the current channel is obtained from pilots, whose transmission degrades the spectral efficiency. Thus, deployed digital receivers are likely to possess small labeled data sets, hardly in the scale needed to train \acp{dnn}. %This paper addresses the problem of small labeled data sets via augmentations. 
Consequently, a core challenge associated with the usage of \ac{dnn}-aided receivers stems from the need to aggregate sufficient task-specific data, i.e., data corresponding to the instantaneous setting where the receiver is required to operate.

%Augmentations refer to techniques that enrich the data set with new synthetic samples, with the augmentations presented in this paper being tailored to the communication domain.

%\subsection{Related Work}
Various strategies have been proposed  to facilitate the application of \acp{dnn}-aided receivers with limited data sets. 
The first approach trains with data obtained from simulations and past measurements and uses the limited data corresponding to the instantaneous channel to estimate some missing parameters, e.g., a channel matrix. These parameters are then used by the network, either as an input \cite{honkala2021deeprx,zhao2021deep} or as part of some internal processing  \cite{he2020model,khani2020adaptive, samuel2019learning, goutay2021machine,pratik2020re}. This  involves imposing a relatively simple model on the channel, typically a linear Gaussian model, which limits their suitability in the presence of complex channel models.  

An alternative approach designs receivers with compact task-specific \acp{dnn} such that they can be trained with relatively small data sets, by integrating them into classic receiver processing via model-based deep learning techniques \cite{shlezinger2020model, shlezinger2022model}, see, e.g., \cite{shlezinger2020data,shlezinger2019deepSIC, shlezinger2019viterbinet,raviv2020data}.
These hybrid model-based/data-driven receivers build on existing communication models and incorporate deep learning into their design, rather than replace the known model altogether with a black-box receiver. The resulting receivers are agnostic to the  channel model and its parameters, imitating the operation of a detection algorithm with no channel knowledge. Although these \ac{dnn}-aided receivers are compact in terms of trainable parameters, the amount of data required in training is still likely to be larger than the amount corresponding to the instantaneous channel one can typically obtain in real-time.

A third approach aims to optimize the training algorithm itself, rather than the architecture, facilitating rapid convergence of the training procedure with limited data.  Optimizing the hyperparameters that govern the optimization process is intuitively seen as a method to share data from different time steps, increasing the effective labeled data sets.
This can be achieved by leveraging  data corresponding to past channel realizations in order to tune the optimization hyperparameters via Bayesian optimization techniques~\cite{wang2021jointly}; model-agnostic meta-learning  \cite{park2020learning,park2020meta,simeone2020learning}; and predictive meta-learning which learns transition patterns in time-varying channels \cite{raviv2022online}. 
%distilling domain knowledge into the training algorithm itself \cite{park2020learning,park2020meta,simeone2020learning,raviv2021meta,raviv2022online}, rather than the architecture, facilitating rapid convergence of the training procedure with limited data. Namely, \ac{maml} \cite{finn2017model} is employed to calculate an inductive bias that allows quick re-training and adaption to different test scenarios, unseen at training time. Optimizing the hyperparameters that govern the optimization process is intuitively seen as a method to share data from different time steps, increasing the effective labeled data sets. Specifically, the method presented in \cite{raviv2022online} is tailored to rapidly time-varying channels, where the channel changes significantly between the consecutive packets.

The aforementioned strategies focus on either the architecture or the training algorithm. A complementary approach to cope with limited data sets, which can be combined with any of the above techniques, is to generate more data at the receiver. Current techniques aim at assigning labels to channel outputs not associated with pilots by exploiting the presence of channel coding for self-supervision \cite{shlezinger2019viterbinet, shlezinger2020inference, shlezinger2019deepSIC,teng2020syndrome} or by using active learning techniques \cite{be2019active, finish2022symbol}. However, these approaches cannot synthesize more data than the block length (typically generating much less \cite{finish2022symbol}), and the resulting data set may be too small for training.

A common practice in the deep learning literature  is to synthesize data samples via {\em data augmentation}. Data augmentation is a set of techniques that enrich a trainable model with new unseen synthetic data, where each technique builds on partial knowledge of the data  characteristics~\cite{shorten2019survey,nalepa2019data,feng2021survey,park2019specaugment}, typically exploiting some underlying translation invariance.  For instance, in image classification~\cite{shorten2019survey,nalepa2019data}, one can use a labeled image to generate multiple different images with the same label by, e.g., rotating or clipping it. While data augmentation is a widely used deep learning technique, it is highly geared towards the common image and language data. This motivates the study of augmentation techniques for enriching data in digital communications, as means to facilitate the training of \ac{dnn}-aided receivers with limited data sets.

\subsection*{Main Contributions}

% highlight our differences from previous or related works
In this paper we propose a data augmentation framework for \ac{dnn}-aided receivers. Our proposed method introduces a set of data synthesis techniques which exploit expected structures of digital communication channel outputs to enrich a small labeled data set with many reliable samples. The resulting enriched data can then be used for training, so as to reduce the error rate obtained by the receiver. 
Our main contributions are summarized as follows: 
\begin{itemize}
    \item \textbf{Proposed framework:} We formulate a communication-directed data augmentations framework, which embodies the specific characteristics of the digital communication data used for training \ac{dnn}-aided receivers.
    \item \textbf{Communications tailored augmentations:} We propose several augmentations that exploit innate traits of digital constellations. We exploit both expected symmetries in channel outputs as well as identified communication-specific translation invariance properties to generate new synthetic samples for training. 
    \item \textbf{Extensive experimentation:} \TomerFill{We extensively evaluate the proposed training scheme for both \ac{siso} and \ac{mimo} systems, considering different channel profiles. We demonstrate consistent benefits by using our approach with various \ac{dnn}-aided receivers, which amounts to gains of up to 3B compared with non-augmented training.} Detail the gains of our scheme once we finish the numerical part.
\end{itemize}

 The rest of this paper is organized as follows:  Section~\ref{sec:system_model} details the system model, while Section~\ref{sec:data_augmentations_static} formulates the frameworks and presents the augmentation techniques for static channels, where a single small data set corresponding to a specific channel realization is to be synthetically enriched for training. Section~\ref{sec:data_augmentations_dynamic} extends the augmentations to dynamic communication setups, accounting for continuous variations in block fading channels. Finally, experimental results and concluding remarks are detailed in Section~\ref{sec:numerical_evaluations} and Section~\ref{sec:conclusion}, respectively.

Throughout the paper, we use boldface letters for vectors, e.g., ${\myVec{x}}$; $({\myVec{x}})_i$ denotes
the $i$th element of ${\myVec{x}}$. %We use upper-case letters for \acp{rv}, and lower-case letters for deterministic quantities. 
Calligraphic letters, such as $\mySet{X}$, are used for sets, 
and $\mySet{R}$ is the set of real numbers.



==> sections/results.tex <==
\section{Numerical Evaluations}
\label{sec:numerical_evaluations}
\vspace{-0.1cm} 
\TomerFill{In this section we numerically evaluate the proposed online adaptation scheme in finite-memory \ac{siso} chanels and in memorylesss multi-user \ac{mimo} setups\footnote{The source code used in our experiments is available at \href{https://github.com/tomerraviv95/data-augmentations-static-channel}{https://github.com/tomerraviv95/data-augmentations-static-channel}}. 
We first describe the receivers compared in our experimental study, detailing the architectures in Subsection~\ref{subsec:simEqualizers} and the training methods in Subsection~\ref{subbsec:Training Methods}. Then, we present the main simulation results for evaluating online meta-learning on linear synthetic channels, non-linear synthetic channels, and channels obeying the COST 2100 model in Subsections~\ref{subsec:synth_simulation_results} to \ref{subsec:cost_simulation_results}. Finally, we numerically evaluate Algorithm~\ref{alg:modular-training} which combines online meta-learning with the modular training in Subsection~\ref{subsec:modular-training}.} From here to conclusions - should replace.
%, as well as the effect of our learning schemes on pilot efficiency, in Subsections~\ref{subsec:modular-training} and \ref{subsec:pilot-training}, respectively.


%-----------------------------------
%	ViterbiNet
%-----------------------------------
% \subsection{ViterbiNet}
% \label{subsec:ViterbiNet}


% Following the channel definition of Subsection~\ref{subsec:SISOChannel}, the Viterbi equalizer solves the maximum likelihood sequence detection problem
% \begin{align}
% \hat{\myVec{s}}_j   
% &= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i,j}\right)\right\}.
% \label{eqn:ML3} 
% \end{align}	
% In particular,  \eqref{eqn:ML3} is solved recursively via dynamic programming, by  iteratively updating a {\em path cost} $c_i(\myStateR)$ for each state $\myStateR\in \bar{\mySet{S}}$ for $i=1,2,\ldots,B$. ViterbiNet implements Viterbi detection in a data-driven fashion by training a \ac{dnn} to provide a parametric estimate of the likelihood function $\hat{P}_{\Weights}\left( \myVec{y}  |  \myStateR\right)$. Meta-ViterbiNet \cite{raviv2021meta} applies Algorithm~\ref{alg:online-meta-learning} to ViterbiNet, leading to higher adaptivity over fast channel variations.

%-----------------------------------
%	Evaluated Equalizers
%-----------------------------------
\vspace{-0.4cm}
\subsection{Evaluated Receivers}
\label{subsec:simEqualizers}
The receiver algorithms used in our experimental study vary based on the considered settings:
%\vspace{-0.1cm}
\subsubsection{Finite-Memory \ac{siso} Channels}
We compare employ ViterbiNet for \ac{siso} settings. The ViterbiNet equalizer, proposed in \cite{shlezinger2019viterbinet}, which is a \ac{dnn}-based Viterbi detector for finite-memory channels of the form \eqref{eqn:ChModel1} \cite{viterbi1967error}. The Viterbi equalizer (from which ViterbiNet originates) solves the maximum likelihood sequence detection problem
\begin{align}
\hat{\myVec{s}}_j   
&= \mathop{\arg \min}_{\myVec{s} \in \mySet{S} }\left\{-\sum\limits_{i=1}^{\Blklen } \log \Pdf{\myVec{Y}_{i,j} | \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}\left( \myVec{y}_{i,j}  |  \myStateR_{i-\Mem+1,j},\ldots, \myStateR_{i,j}\right)\right\}.
\label{eqn:ML3} 
\end{align}	
ViterbiNet computes each log likelihood using a  \ac{dnn} that requires no  knowledge of the channel  distributions $ \Pdf{\myVec{Y}_j |  \myState_{i-\Mem+1,j},\ldots, \myState_{i,j}}$. This internal \ac{dnn} is implemented using three fully-connected layers of sizes $1\times 100$, $100\times 50$, and $50 \times |\mySet{S}|^\Mem$, with activation functions set to sigmoid (after first layer), ReLU (after second layer), and softmax output layer.

\subsubsection{Memoryless \ac{mimo} Channels}
We evaluate the DeepSIC receiver detailed in Subsection~\ref{subsec:modular_training_example}. The building blocks of DeepSIC are implemented using three fully-connected layers:  An $(N + K - 1) \times 100$ first layer, a $100 \times 50$ second layer, and a $50 \times |\mySet{S}|$ third layer, with a sigmoid and a ReLU intermediate activation functions, respectively. The number of iterations is set to $Q=5$.

Each receiver is trained by the adam optimizer with learning rate of $1e^(-3)$.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_train_channel.png}
    \caption{Synthetic training channel.}
    \label{fig:synthetic_train_channel}
    \end{subfigure} 
    %
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_test_channel.png}
    \caption{Synthetic test channel.}
    \label{fig:synthetic_test_channel}
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.31\textwidth}
    \includegraphics[width=\textwidth,height=0.15\textheight]{fig/cost_channel.png}
    \caption{COST 2100 channel.}
    \label{fig:COSTChannel} 
    \end{subfigure}
    \caption{Examples of time-varying channels: channel coefficients versus block index.}
    \figSpace
    \label{fig:channels} 
 %   \vspace{-0.1cm}
\end{figure*}

\subsection{Augmentations Methods}
\label{subsec:evaluated_augmentations_methods}
We employ the various augmentations discussed in Section \ref{sec:data_augmentations_static}, as well as the next baseline methods:
\begin{itemize}
    \item {\em Regular training}: No augmentations are applied; the \ac{dnn} is trained using solely the pilots.
    \item {\em Extended pilot training}: Transmitting 3x times the pilot size, and training regularly without augmentations.
    \item {\em Partial knowledge (PK) augmentation}: A genie-aided scheme that knows the instantaneous channel taps, and uses it to estimate the noise realizations.
    Then, it synthesizes $K$ words per class by generating a random symbols word, convolve it with the  taps and add the estimated noise.
    \item {\em Full knowledge (FK) augmentation}: A genie-aided scheme that knows the instantaneous channel taps and the \ac{snr}, and synthesizes $K * 2^\Mem$ words at each step of training. This schemes serves as a lower-bound on the achievable \ac{ber}.
\end{itemize}

%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{Linear Synthetic Channel Results}
\label{subsec:synth_simulation_results}
\vspace{-0.1cm}
We begin by evaluating Algorithm~\ref{alg:online-meta-learning} on synthetic time-varying linear channels with additive Gaussian noise, considering  a finite-memory \ac{siso} setting and a memoryless \ac{mimo} setup.
%
\subsubsection{\ac{siso} Finite-Memory Channels} 
We transmit $\Blklen_p=100$ pilots followed by $\Blklen_p=5000$ data bits, for a total transmission of a single block with size $\Blklen=\Blklen_p+\Blklen_d=5100$. This means that only a small number of pilots are used to estimate the concurrent channel. We consider a linear Gaussian channel, whose input-output relationship is given by
\begin{equation}
\label{eqn:Gaussian}
\myY_{i,j} = \sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j},
\end{equation}
where $\myVec{h}_j = [h_{0,j},\ldots,h_{\Mem-1,j}]^T$ are the real channel taps, and $w_{i,j}$ is \acl{awgn} with variance $\sigma^2$. The channel memory is $\Mem = 4$ with the taps $\{h_{l,j}\}$  generated using a synthetic model representing oscillations of varying frequencies. 
%
Here,  the signals received during the pilots used for initial training $(\mathcal{D}_0)$ are subject to the time-varying channel whose taps are illustrated in Fig.~\ref{fig:synthetic_train_channel}; while we use the taps  in Fig.~\ref{fig:synthetic_test_channel} for testing. This channel represents oscillations of varying frequencies. %, where  the periods of the taps become aligned as the noise subsides. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/linear_channel_siso_coded_ber_versus_snrs.png}
    \caption{\ac{siso} - \ac{ser} vs. SNR.}
    \label{fig:linear_synthetic_siso_BER_vs_SNR}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/linear_channel_mimo_coded_ber_versus_snrs.png}
    \caption{\ac{mimo} - \ac{ser} vs. SNR.}
    \label{fig:linear_synthetic_mimo_BER_vs_SNR}
    \end{subfigure}
    %
    \caption{Synthetic linear Gaussian channel.}
    \label{fig:linear_synthetic_BER_vs_SNR} 
    \figSpace
\end{figure*}

In Fig.~\ref{fig:linear_synthetic_siso_BER_vs_SNR} we plot the average \ac{ser} of the considered receiver in conjunction with the various augmentations, when the \ac{snr}, defined as $1/\sigma^2$, is set to values in the range of $9$ dB- $13$ dB. Each point is averaged over 50 trials, to reduce the Monte Carlo estimation noise. Fig.~\ref{fig:SyntheticBERvsBlock} shows that the combined approach significantly outperforms its benchmarks, demonstrating gains of the proposed online meta-learning training and its suitability when combined with receiver architectures utilizing relatively compact \acp{dnn}. In particular, it is demonstrated that each of the ingredients combined in Meta-VitebiNet, i.e., its model-based architecture, the usage of self-supervision, and the incorporation of online meta-learning, facilitates operation in time-varying conditions: The ViterbiNet architecture consistently outperforms the black-box \ac{lstm} classifier; Online training yields reduced \ac{ber} as compared to joint learning; and its combination with meta-learning via Algorithm~\ref{alg:online-meta-learning} yields the lowest \ac{ber} values.  
%
To further validate that these gains also hold for different \acp{snr}, we show in Fig.~\ref{fig:SyntheticBERvsSNR} the average coded \ac{ber} of the evaluated receivers after 300 blocks, averaged over 5 trials. We observe in Fig.~\ref{fig:SyntheticBERvsSNR} that for \ac{snr} values larger than $8$ dB, Meta-ViterbiNet consistently achieves the lowest  \ac{ber} values among all considered data-driven receivers, with gains of up to 0.5dB over the online training counterpart.

\subsubsection{Memoryless MIMO Channels} 
For the \ac{mimo} setting, use $T_p=T_d=50$ blocks. The block length is set to $\Blklen = 152$ symbols, encoding 120 information bits with \acl{rs} [19,15] code. The input-output relationship of a the memoryless Gaussian \ac{mimo} channel is given by
\begin{equation}
\label{eqn:GaussianMIMO}
\myY = \myMat{H}\myS + \myVec{W},
\end{equation}
where $\myMat{H}$ is a known deterministic $N\times K$ channel matrix, and $\myVec{W}$ consists of $N$ i.i.d Gaussian \acp{rv}.  
We set the number of users and antennas to $N=K=4$. The channel matrix $\myMat{H}$ models spatial exponential decay, and its entries are given by
$\left( \myMat{H}\right)_{n,k} = e^{-|n-k|}$, for each $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$.  The transmitted symbols are generated from a \ac{bpsk} constellation in a uniform i.i.d. manner, i.e., $\mathcal{S}=\{\pm 1\}$.

\vspace{-0.4cm}
\subsection{Non-Linear Synthetic Channel Results}
\label{subsec:syntNL_simulation_results}
\vspace{-0.1cm}
Next, we evaluate the proposed online meta-learning scheme in non-linear synthetic channels, where one can greatly benefit from the model-agnostic nature of \ac{dnn}-based receivers. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/linear_channel_siso_coded_ber_versus_snrs.png}
    \caption{\ac{siso} - \ac{ser} vs. SNR.}
    \label{fig:linear_synthetic_siso_BER_vs_SNR}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/linear_channel_mimo_coded_ber_versus_snrs.png}
    \caption{\ac{mimo} - \ac{ser} vs. SNR.}
    \label{fig:linear_synthetic_mimo_BER_vs_SNR}
    \end{subfigure}
    %
    \caption{Synthetic linear Gaussian channel.}
    \label{fig:linear_synthetic_BER_vs_SNR} 
    \figSpace
\end{figure*}

\subsubsection{\ac{siso} Finite-Memory Channels} To check the robustness of our method in a non-linear case, we generate a non-linear channel by applying a non-linear transformation to synthetic channel in \eqref{eqn:Gaussian}. The resulting finite-memory \ac{siso} channel is give by
\begin{equation}
\label{eqn:Gaussian1}
\myY_{i,j} =\tanh{\Big(C \cdot \Big(\sum_{l=0}^{\Mem-1} h_{l,j}S_{i-l,j} + w_{i,j}\Big)\Big)}.
\end{equation}
This operation may represent, e.g., non-linearities induced by the receiver acquisition hardware. The hyperparameter $C$ stands for a power attenuation at the receiver, and chosen empirically as $C=\frac{1}{2}$. All other hyperparameters and settings are the same as those used in the previous subsection. This simulation shows a consistent gain of around $0.75$dB over the SNRs with values of $8$dB - $12$dB, as observed in Fig.~\ref{fig:NonLinearSyntheticBERSISO}.

\subsubsection{Memoryless \ac{mimo} Channels} Similarly to the \ac{siso} case, we simulate a non-linear \ac{mimo} channel from \eqref{eqn:GaussianMIMO} via
\begin{equation}
\label{eqn:Gaussian2}
\myY = \tanh{\Big(C \cdot\Big(\myMat{H}\myS + \myVec{W}\Big)\Big)},
\end{equation}
with $C=\frac{1}{2}$ and the remaining simulation settings are chosen as in Subsection~\ref{subsec:synth_simulation_results}. The numerical results for this channel are illustrated in Fig.~\ref{fig:NonLinearSyntheticBERMIMO}, showing that the superiority of our approach is maintained in non-linear setups. The right part shows an average over 20 trials, while the left graph corresponds to an exemplary trial. In particular, we note that gains of up to 0.5dB in high SNRs are achieved compared with online training, while the gap from joint method is around 0.25dB. Here, our gain becomes apparent as the SNR increases.

==> sections/static.tex <==
\section{Data Augmentations for Static Channels}
	\label{sec:data_augmentations_static}
	\vspace{-0.1cm}
Here, we present the proposed data augmentation techniques, considering a static setting, where one has access to a small data set corresponding to a single channel realization where it should also infer.
In Subsection~\ref{subsec:main_pillars} we introduce the rationale for using augmentations, and discuss the main pillars for data augmentation techniques in light of the operation of \ac{dnn}-aided communication receivers. We follow up with the communication-oriented augmentations in  Subsection~\ref{subsec:augmentations_static}, and provide a discussion in  Subsection~\ref{subsec:discussion}.  

%-----------------------------------
%	Main Pillars
%-----------------------------------
\vspace{-0.4cm}
\subsection{Rationale}
\label{subsec:main_pillars}

Data augmentation is a widely spread practice in machine learning. % for enriching a data set and for encouraging a trainable model to learn some known property of the data. 
For example, in speech processing, data augmentation includes several domain-tailored transforms such as time warping and frequency masking \cite{park2019specaugment}, which use observed sequences to generate new sequences the system should learn to cope with. In general, the purpose of using augmentations is to enrich the data set by exploiting domain knowledge regarding the nature of the data. The enriched set is then used for training the model with samples that may be observed during inference but are not included in the train set.

In digital communications, one is often faced with scarce data scenarios corresponding to a given task, i.e., when one has access to short packets which reflect on the channel coefficients at a specific time. As such, augmentations for communication applications can aid in obtaining new data for training \ac{dnn}-aided receivers. However, existing data augmentation techniques are highly geared towards structures and invariances exhibited by data in conventional machine learning domains such as visual, language, and speech data, and thus cannot be directly implemented in digital communications. 

% TODO NIR CONTINUE FROM HERE - what we discuss here are requirements and not really properties


% Therefore, in order 
% Our communication-oriented approach is differentiated from standard augmentations as it satisfies the following properties:
In the following sections, we develop augmentation techniques for data used by digital receivers.  Our approach accounts for the following data augmentation considerations:
\begin{enumerate}[label={\em C\arabic*}]
    \item \textbf{Domain-oriented} - \label{itm:domain} Data augmentations are inherently domain-oriented \cite{nooraiepour2021hybrid}. In our case, we exploit the inherent structure of digital constellations to formulate class-preserving transformations. 
    \item \textbf{Diversity} - \label{itm:diversiy}  The number of classes grows quickly with the system parameters such as the constellation size and the number of users. As such, the number of samples per class should be kept approximately uniform and above some minimal threshold to avoid class imbalances \cite{be2019active,finish2022symbol}.
    \item \textbf{Complexity} - \label{itm:complexity} As data augmentation is to be implemented by a digital receiver in real-time, we must keep the sample-complexity low and the computation lightweight. 
\end{enumerate}

\begin{figure*}  % spans both columns
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/constellation.pdf}
\caption{Constellation points and received pilots}
\label{fig:constellation}
\end{subfigure}
\hfill % maximize the horizontal distance between the graphs
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/geometric.pdf}
\caption{Geometric augmentation}
\label{fig:geomtric}
\end{subfigure}

\bigskip  % some extra vertical whitespace
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/translation.pdf}
\caption{Translation augmentation}
\label{fig:translation}
\end{subfigure}
\hfill % maximize the horizontal distance between the graphs
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/rotation.pdf}
\caption{Constellation-conserving rotation}
\label{fig:rotation}
\end{subfigure}

\caption{Augmentations exemplified on QPSK constellation} % Overall figure caption
\end{figure*}

% This is achieved by clustering the data based on the constellation symbol, and by adapting this clustering between blocks in block-fading channels as a form of temporal smoothing \cite{cambe2020exploring}.
%-----------------------------------
%	Augmentations
%-----------------------------------
\vspace{-0.4cm}
\subsection{Augmentations}
\label{subsec:augmentations_static}
%to design augmentation mechanisms, one must first identify th properties in digital communications data which can be exploited to synthesize new data. 

% \textcolor{red}{before going into the actual techniques, we should start with how we designed it. Particularly, what kind of models guide us in our design? We need to begin with a description of the following flavour:\\
% We draw our inspiration from common wireless communication models, where: \\
% 1. The channel output is often corrupted by additive distortion, e.g., noise and interference, which does not depend on the transmitted symbols. Thus we can often write $\myVec{y} = g(\myVec{s}) + \myVec{d}$ where $\myVec{d}$ is the additive distortion term that is invariance of $\myVec{s}$, and $g(\cdot)$ is the channel mapping capturing, e.g., the propagation environment between the transmitter and the receiver. This observation is what motivates our geometric augmentation and our translation augmentation. \\
% 2. Many constellations are symmetric, and thus there exist a discrete set of linear transformations which are constellation preserving, i.e., for every positive integer $n$ these exists a set of $n\times n$ matrices $\{\myMat{P}_i\}$ such that if  $\myVec{s}\in\mySet{S}^n$, it holds that   $\myMat{P}_i\myVec{s}\in\mySet{S}^n$ for each $i$. However, the channel mapping $g(\cdot)$  is not invariant to any such constellation preserving translation, and thus to build upon this property for augmentation one must  identify translations that are likely to be preserved by $g(\cdot)$. \\
% After we have this description, we can describe the following augmentation based on these properties and in light of considerations \ref{itm:domain}-\ref{itm:complexity}}

Designing communication-specific augmentations requires one to identify label-invariant transformations that must account for the statistical model, being the underlying input-output relationship induced by the communication model in our case. In the following, we detail three different and complementary augmentations: (1) geometric augmentation; (2) translation augmentation; and (3) constellation-reserving rotation. Each of these methods  originates from some expected wireless-communication behaviour.

\subsubsection{Geometric Augmentation} 
Our first augmentation technique draws inspiration from the common model of wireless channels as being decomposable into a channel response and an additive noise term. In such cases, one can write
\begin{equation}
    \label{eqn:addNoiseChannel}
    \myVec{y}=g(\myVec{s})+\myVec{d},
\end{equation}
where $g$ is the channel input-to-output transformation, and $\myVec{d}$ is an additive distortion term which is independent of $\myVec{s}$, e.g., thermal noise and interference.  This representation indicates that channel outputs corresponding to the same input tend to form clusters, as illustrated in Fig.~\ref{fig:constellation}, where the intra-cluster distribution is invariant of the center, as the noise is independent of the  signal. 
This geometrical interpretation of the by-class clusters can be employed to generate additional class-specific data.

In particular, we propose to use the existing labeled data $\mySet{Q}$ to identify clusters in the observations space from which the received symbols are likely to originate. Our method is based on clustering the channel outputs in $\mySet{Q}$ and setting $\myVec{\mu}$  and $\myMat{\Sigma}$ to be the cluster-wise centers and covariances, respectively.  %We characterize each cluster using its estimated first and second order statistical moments, which are estimated from the available data.
%empirically to cluster all received patterns per class via a Gaussian distribution. Each class distribution is dictated by two parameters, cluster center and its variance, both learned from the available pilots data.
%
Using the identified clusters, we suggest to synthesize data corresponding to a constellation point $\mypoint$ from a conditional Gaussian distribution $\mathcal{N}(\myVec{\mu}(\mypoint),\,\myMat{\Sigma}(\mypoint))$. 

Therefore, in order to enrich a labeled data set $\mySet{Q}$ into $\mySet{Q}^*$, we use $\mySet{Q}$ to determine $\myVec{\mu}$  and $\myMat{\Sigma}$ for each $\mypoint$. To that aim, we define the index set corresponding to $\mypoint$ as 
\begin{equation}
    \label{eqn:IdxSet}
    \mySet{I}_{\mySet{Q}}(\mypoint) := \{i| \mystate_i \in \mySet{Q}; \mystate_i =  \mypoint \}.
\end{equation}
We can now  estimate the moments of the clusters as
 \begin{equation} \label{eq:mean_calculation}
    \myVec{\mu}(\mypoint) =\frac{1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \myVec{y}_{i},
\end{equation}
and similarly 
 \begin{equation} \label{eq:variance_calculation}
    \!\!\myMat{\Sigma}(\mypoint) \!=\!\frac{1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \!\!\!\!(\myVec{y}_{i}\! - \!\myVec{\mu}(\mypoint))(\myVec{y}_{i} \!-\! \myVec{\mu}(\mypoint))^T.
\end{equation}
To avoid empty sets $\mySet{I}(\mypoint)$, one can opt pilot sequences for which each class has at least a single representative. The augmentation is depicted in Fig.~\ref{fig:geomtric}.
 %
Once the clusters are set, they are used to draw synthetic samples $\myVec{y}^{\prime}$ for some corresponding label $\mypoint^{\prime}$. %The tuple $(\myVec{y}^{\prime},\mypoint^{\prime})$ is the input to the next augmentation. 
  
\subsubsection{Translation Augmentation} 
In the previous augmentation we exploited labeled data to generate new samples for a single constellation point. To extend this notion, the current augmentation aims to share data across different clusters. Here, we again build upon the additive distortion model in \eqref{eqn:addNoiseChannel}, and instead of generating new samples around a given cluster in a random fashion, we estimate the {\em realization} of the distortion. We thus leverage the assumption that the distortion is independent of the transmitted symbols, and use its estimate to generate samples from other clusters.

%\textcolor{blue}{To formulate this notion, let us take a commonly used model that assumes a channel output that is corrupted by additive distortion, e.g., noise and interference, which does not depend on the transmitted symbols. Thus, we can write $\myVec{y} = g(\myVec{s}) + \myVec{d}$ with $\myVec{d}$ being the additive distortion term that is invariant of the class $\myVec{s}$, and with $g(\cdot)$ being the channel mapping that captures the propagation environment between the transmitter and receiver. As the additive term $\myVec{d}$ is class-invariant, estimation of its value for a first class, also approximately holds for a second class. This observation is what motivates our translation augmentation.}. To that end, we translate geometric-augmented data points between different clusters. 

%\textcolor{red}{can we describe this in a way which does not divide whether SISO or MIMO? can we just use the general formulations of $\myVec{y}$ and $\myVec{s}$?}

To formalize this idea, consider a labeled pair $(\myVec{y},\mypoint)$, and let $ \myVec{\mu}(\mypoint)$ be the cluster center estimated in the previous scheme. We now introduce the difference vector $\hat{\myVec{d}}$, which measures the difference between the channel output and the empirical cluster center, i.e.,
\begin{equation} \label{eq:difference_calculation}
    \hat{\myVec{d}} =\myVec{y} - \myVec{\mu}(\mypoint)
\end{equation}
and randomly choose a constellation point $\mypoint^{\prime}$ that is different from $\mypoint$. Then, we can generate an additional sample by adding the difference to the calculated cluster center of $\mypoint^{\prime}$. Namely, we compute
\begin{equation} \label{eq:difference_addition}
     \myVec{y}^{\prime} = \myVec{\mu}(\mypoint^{\prime}) + \myVec{d},
\end{equation}
to obtain the augmented pair $(\myVec{y}^{\prime},\mypoint^{\prime})$, as illustrated in Fig.~\ref{fig:translation}.

\subsubsection{Constellation-Conserving Rotations} 
Many constellations are symmetric by design. This means that there exists a discrete set of linear transformations $\{\myMat{P}_u\}$ which are \textit{constellation-conserving}. A $\Blklen \times \Blklen$ matrix $\myMat{P}_u$ represents a constellation-conserving transformation if for every $\myVec{s}\in\mySet{S}^\Blklen$, it is satisfied that $\myMat{P}_u\myVec{s}\in\mySet{S}^\Blklen$ as well. This property may be exploited to generate additional training data when it meets the following two requirements:
\begin{itemize}
    \item The distribution of the noise is invariant to the transformation, i.e., that $\myMat{P}_u\myVec{d}$ obeys (approximately) the same distribution as  $\myVec{d}$.
    \item The channel mapping $g(\cdot)$ in \eqref{eqn:addNoiseChannel} (approximately) satisfies $\myMat{P}_u g(\myVec{s}) \approx g(\myMat{P}_u \myVec{s})$.
\end{itemize}
When the above hold, one can use a labeled pair $(\myVec{y}, \myVec{s})$ to generate additional data $(\myVec{y}^\prime, \myVec{s}^\prime)$ by noting that
\begin{equation}
\myVec{y}^\prime =\myMat{P}_u\myVec{y} = \myMat{P}_u g(\myVec{s}) + \myMat{P}_u\myVec{d} \approx  g(\myMat{P}_u\myVec{s}) + \myMat{P}_u\myVec{d}, 
\end{equation}
which is approximately identically distributed as an output obtained from the channel input $\myVec{s}^\prime = \myMat{P}_u\myVec{s}$.

% by applying it to the simplified model $\myMat{P}_u\myVec{y} = \myMat{P}_u g(\myVec{s}) + \myMat{P}_u\myVec{d}$ with two main requirements. First, we demand the distortion to be transformation-agnostic $\myMat{P}_u\myVec{d} \approx \myVec{d}$. Second, we assume  Under these requirements, the tuple $(\myMat{P}_u \myVec{y},\myMat{P}_u \myVec{s})$ may be added to the augmented batch for training. 

% TODO NIR CONTINUE FROM HERE
To design constellation-preserving augmentations, we note that communication channel mappings are often commutative to scalar multiplication, i.e., $g(\alpha \myVec{s}) = \alpha g(\myVec{s})$ for scalar $\alpha$. This holds for instance, when the channel is linear. Consequently, we focus on the discrete rotations transformations, for which $\myMat{P}_{u} = e^{j \pi \frac{\phi_u}{180}} \myMat{I}$. Under an M-PSK constellation, for example, one can set $\phi_u = \frac{2\pi u}{M}$ for any $u \in \{1,\ldots,M-1\}$ while having that $\myMat{P}_{u}\myVec{s}$ is a valid constellation vector. Furthermore, the distribution of noise signals is often rotation-invariant as is the case for, e.g., circularly-symmetric Gaussian $\myVec{d}$. Consequently, permutations of such case are likely the be constellation-preserving and satisfy the above requirements. 

\textcolor{red}{we should formulate each part separate as if it starts from the $\mySet{Q}$ and updates it into $\mySet{Q}^\star$.}

The resulting proposed augmentation operates as follows: First, we denote the set of constellation-conserving rotations by $\{\myMat{P}_{u}\}$. Then, we choose a random $\myMat{P}_{u}$ and multiply the corresponding phase with the translation-augmented pair: 
\begin{equation} \label{eq:constellation_conserving_rotation}
     \myVec{y}^{\prime\prime\prime} = \myMat{P}_{u} \myVec{y}^{\prime\prime},\quad 
     \mypoint^{\prime\prime\prime} = \myMat{P}_{u} \mypoint^{\prime\prime}.
\end{equation}
The final augmented pair $(\myVec{y}^{\prime\prime\prime},\mypoint^{\prime\prime\prime})$ is added to the buffer $\mySet{Q}^*$. See an illustration of a synthetic example in Fig.~\ref{fig:rotation}.

\subsubsection{Combined Scheme} 
Each of the aforementioned methods allows to generate additional new data from an available labeled set comprised of channel outputs and their corresponding transmitted symbols. As these methods are complementary of each other, we combine them into an overall data augmentation method  by applying them subsequently.  

First, we initialize the buffer by $\mySet{Q}^*=\mySet{Q}$. To realize the diversity consideration \ref{itm:diversiy}, we draw $K$ samples from each class distribution, which goes through the augmentation pipeline. Then, we add all synthetic samples to the augmented training batch $\mySet{Q}^*$, resulting in a set of $|\mySet{Q}| + K\cdot M$ labeled samples to be used for training $\Weights$, as illustrated in Fig.~\ref{fig:transmission}. Note the each augmentation may be applied on its own, or in consecutive pairs. However, we provide empirical demonstration in Section~\ref{sec:numerical_evaluations} that augmented pairs that are the output of two different augmentations are usually independent of each other, causing the gain from each augmentation to sum up. The resulting combined augmentation policy $\psi_{static}:\mySet{Q} \mapsto \mySet{Q}^*$ for static channels is formulated in full as Algorithm~\ref{alg:StaticAugmentationScheme}.

\begin{figure}
  \begin{algorithm}[H]
    \caption{Static Channel Augmentation Scheme $\psi_{static}$}
    \label{alg:StaticAugmentationScheme}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwFor{RepTimes}{repeat}{times}{end}
    \SetKwProg{AugmentationScheme}{Augmentation Scheme}{}{}
    \Input{data set $\mySet{Q}$; \newline total number of augmented samples $K$} %  \newline 
 %   \Output{augmented batch $\mySet{Q}^*$}
    \AugmentationScheme{$(\mySet{Q},K)$}{
        $\myVec{\mu}(\mypoint) \gets$ calculate by  \eqref{eq:mean_calculation}, $\forall \mypoint \in \mySet{S}^L|\mySet{S}^K$\;\label{line:centers_calculation}
        
        $\myMat{\Sigma}(\mypoint) \gets$ calculate by  \eqref{eq:variance_calculation}, $\forall \mypoint \in \mySet{S}^L|\mySet{S}^K$\;\label{line:variance_calculation}

    Initialize $\mySet{Q}^* = \mySet{Q}$\;
    \For{$\mypoint^{\prime}$ in $\mySet{S}^L|\mySet{S}^K$}{%
                \RepTimes{K}{
                \nonl\texttt{Geometric Augmentation}\;

                sample $\myVec{y}^{\prime}$ from $\mathcal{N}(\myVec{\mu}(\mypoint),\,\myMat{\Sigma}(\mypoint))$;\label{line:sample_from_distribution}
                
                \nonl\texttt{Translation Augmentation}\;
                
                $\myVec{d} \gets$ calculate by  \eqref{eq:difference_calculation}\;\label{line:difference_calculation}
                
                sample $\mypoint^{\prime\prime}$ from $\mySet{S}^L|\mySet{S}^K/\mypoint^{\prime}$\;\label{line:constellation_sampling_second}
                
                $\myVec{y}^{\prime\prime} \gets$ calculate by  \eqref{eq:difference_addition}\;\label{line:difference_addition}
                
                \nonl\texttt{Constellation-Conserving Rotation}\;
                
                choose a random $\myMat{P}_{u}$\;
                
                $\myVec{y}^{\prime\prime\prime},\mypoint^{\prime\prime\prime} \gets$ rotation by \eqref{eq:constellation_conserving_rotation}\;
                
                \nonl\texttt{Buffer update}\;
                add $(\myVec{y}^{\prime\prime\prime},\mypoint^{\prime\prime\prime})$ to buffer $\mySet{Q}^*$; \label{line:add_to_buffer}
                
                }}
        \KwRet{$\mySet{Q}^*$}
  }
  \end{algorithm}
\end{figure}

%-----------------------------------
%	Discussion
%-----------------------------------
\vspace{-0.4cm}
\subsection{Discussion}
\label{subsec:discussion}

Algorithm~\ref{alg:StaticAugmentationScheme} integrates data augmentation into digital receiver processing, synthesizing channel outputs data from the input pilots. This data allows the receiver to train without relying on lengthy pilot transmissions, achieving accurate training with short pilots as empirically demonstrated in Section~\ref{sec:numerical_evaluations} and increasing the effective transmitted pilots size. The suggested  policy differs from augmentations in other domains, e.g., vision, being specifically tailored to communications. This domain knowledge includes the geometrical interpretation of the channel outputs which follows from the typical arrangements of digital constellations; the expected balanced symbol diversity as communication symbols are typically uniformly distributed; and the symmetry of common constellations. in the following section we show how one can also incorporate knowledge regarding the continuous operation of digital receivers, which allows to benefit from the presence of past channels and data, while also restricting to framework to light computations. Contrary to other domains, where augmentations often rely on complex policies, e.g., using generative networks \cite{almahairi2018augmented} or reinforcement learning \cite{laskin2020reinforcement}, we keep our mechanism light. The operations required for our scheme include: sampling from a Gaussian distribution, adding and subtracting vectors and lastly multiplying by a phase. These operations allow our mechanism to be carried out in real time.

Algorithm~\ref{alg:StaticAugmentationScheme} can be combined with other approaches for training deep receivers with scarce data. These approaches include the model-based methods \cite{shlezinger2020model}, as well as self-supervision methods \cite{finish2022symbol,shlezinger2019viterbinet}, which assign decision-directed labels to  channel outputs and uses them for training. While self-supervision cannot generate more samples than the block length, Algorithm~\ref{alg:StaticAugmentationScheme} can synthesize any number of samples, and is thus suitable for coping with short block lengths. 


==> sections/system_model.tex <==
\section{System Model}
\label{sec:system_model}
\vspace{-0.1cm}

In the section, present the system model. To that aim, we first describe the communication model in Subsection~\ref{subsec:communication_model}, and the we discuss the receiver processing and the considered problem formulation of data augmentation for \ac{dnn}-aided receivers in Subsection~\ref{subsec:Receiver}. 

%-----------------------------------
%	Communication Model
%-----------------------------------
\vspace{-0.2cm}
\subsection{Communication Model}
\label{subsec:communication_model}
\vspace{-0.1cm} 
We consider a generic digital communication system in discrete-time. 
Let $\myVec{s}_i\in\mySet{S}$ be a symbol transmitted from constellation $\mySet{S}$ (with its size denoted $|\mySet{S}|$) at the $i$th time instance, $i \in \{1,2,\ldots, \Blklen\}$. The input block $\mys := \{\myVec{s}_i\}_{i\in \Blkset}$ is divided into $\Blklen_{\rm pilot}$ pilots that are known to the receiver,  denoted $\myVec{s}^{\rm pilot}$, and  $\Blklen_{\rm info} = \Blklen-\Blklen_{\rm pilot}$ information symbols $\myVec{s}^{\rm info}$ that are unknown. The channel output at time instance $i$ is denoted by $\myVec{y}_i$ which take value in some set $\mySet{Y}$, and the received block is $\myVec{y}:= \{\myVec{y}_i\}_{i\in \Blkset}$. It can be separated by the receiver, similarly as the channel input, into its pilot and information parts denoted $\myVec{y}^{\rm pilot}$ and $\myVec{y}^{\rm info}$, respectively. We assume that the channel, i.e., the mapping from $\myVec{s}$ into $\myVec{y}$, is constant within a block of $\Blklen$ channel uses, which thus corresponds to the coherence duration of the channel. 

{\bf Channel Models:} 
While the above channel model is generic, we focus mostly on the common setting of communication over casual finite-memory channels. 
We note two important cases of this channel model, which are also the ones considered in our experimental study:
\begin{enumerate}
    \item \emph{\ac{siso} Finite-Memory Channels}: In multipath \ac{siso} channel, the channel output $\myVec{y}_{i}$ depends on the last $\Mem > 0$ transmitted symbols, where $\Mem$ is the memory length, and is given by a stochastic function of the last $\Mem$ transmitted symbols $\mystate_i := [\myVec{s}_{i-\Mem+1},\ldots, \myVec{s}_{i}]^T \in \mySet{S}^L$.  
    Specifically, the conditional distribution of the channel output given its input satisfies   
    \begin{equation}
    	\label{eqn:ChModel1}
    	P\left(\myVec{y} | \myVec{s} \right)  = 
    	\prod\limits_{i\!=\!1}^{\Blklen}P\left(\myVec{y}_i |\mystate_i\right).  
    \end{equation}
    %In \eqref{eqn:ChModel1}, the lower-case notations $\myVec{s}$, $\myVec{y}_i$, and $\myStateR_i$ represent the realizations of the \acp{rv} $\myS$, $\myY_i$, and $\myState_i$, respectively. 
    We set $\myVec{s}_i \equiv \myVec{0}$ for $i<0$, i.e., we assume a guard interval of at least $\Mem-1$ time instances prior to the beginning of the block. %In this case, $\mystate_i \in \mySet{S}^L$ and $\myVec{y}_i\in \mySet{Y}$. 
    \item \emph{Flat \ac{mimo} Channels}: Another channel of interest is the memoryless \ac{mimo} channel, where $\myVec{s}_i \in \mySet{S}^K$ and $\myVec{y}_i \in \mySet{Y}^N$ with $K>1$ and $N>1$. The variable $K$ denotes the number of single-antenna transmitters, and for $K>1$ the setting represents a multiple access channel. The variable $N$ represents the number of receive antennas. %We denote $\mystate_i \equiv \myVec{s}_i$ in this case, for ease of notation.
\end{enumerate}
%For both channels, one can replace $\myVec{s}_i$ with $\mystate_i$ in \eqref{eq:meta_1}, \eqref{eqn:ErrorRate} and in $\mySet{Q}= \{(\myVec{y}_i^{\rm pilot},\mystate_i^{\rm pilot}) \}$.

%-----------------------------------
%	Receiver
%-----------------------------------
\vspace{-0.2cm}
\subsection{Receiver Operation and Problem Formulation}
\label{subsec:Receiver}
\vspace{-0.1cm} 
The receiver processing is aided by a  \ac{dnn} which relies on labeled data to learn its mapping. In particular, the receiver recovers the information symbols from $\myVec{y}^{\rm info}$ using a \ac{dnn}-aided detection mapping, which yields the estimate $\hat{\myVec{s}}(\myVec{y}^{\rm info}; \Weights)$, where  $\Weights$  are the  parameters of the \ac{dnn}.
The parameters $\Weights$ are obtained by training, using the available labeled data representing the underlying channel which is denoted by $\mySet{Q}^*$.
The training module follows a (stochastic) gradient-based optimization with empirical loss measure $\mySet{L}_{\mySet{Q}^*}$, e.g., iterations of the form
 \begin{align}
\label{eq:local_update} % \label{eq:meta_1}
\Weights^{(t+1)} = \Weights^{(t)} - \eta \hat{\nabla}_{\Weights}\mySet{L}_{\mySet{Q}^*}(\Weights^{(t)}),
 \end{align}
 where $\eta > 0$ is the learning rate and $\hat{\nabla}_{\Weights}\mySet{L}$ is a stochastic approximation of the gradient of the empirical loss with respect to the trainable parameters. Since symbol detection is a classification task, we focus on $\mySet{L}_{\mySet{Q}^*}$ being the empirical cross-entropy loss, such that \eqref{eq:local_update} approximates the solution to
 \begin{align}
\label{eq:meta_1}
  \mathop{\arg \min}_{\Weights} \Big\{ \mySet{L}_{\mySet{Q}^*}(\Weights) = -\sum_{(\myVec{y}_i, \myVec{s}_i) \in\mySet{Q}^* }\log \hat{P}_{\Weights}\left(\myVec{s}_{i}|\myVec{y}_{i} \right)\Big\},
\end{align}
with $\hat{P}_{\Weights}(\cdot|\cdot)$ representing the soft (probabilistic) estimates produced by the receiver with \ac{dnn} parameters $\Weights$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/communication scheme.PNG}
    \caption{System model illustration.}
    \label{fig:transmission}
\end{figure}

While the \ac{dnn}-aided receiver trains with a labeled data set for which the transmitted symbols are known, its performance is measured in its ability to recover the information data. Consequently, the considered performance measure for evaluating the parameters $\Weights$ trained via \eqref{eq:local_update} is the error rate over the information block 
\begin{equation}
\label{eqn:ErrorRate}
	e(\Weights) = \frac{1}{\Blklen_{\rm info}}\sum_{i=1}^{\Blklen_{\rm info}} \Pr\left( \hat{\myVec{s}}_i(\myVec{y}^{\rm info};\Weights) \neq  \myVec{s}_i^{\rm info} \right). 
\end{equation} 
An illustration of the system is depicted in Fig.~\ref{fig:transmission}.

{\bf Problem Formulation:} 
Note that the labeled data set corresponding to the current channel to which the receiver has access is  $\mySet{Q}= \{(\myVec{y}_i^{\rm pilot},\myVec{s}_i^{\rm pilot}) \}$, i.e., the known pilots and their respective received values.  When the number of samples $B_{\rm pilot}$ is relatively small, training via \eqref{eq:local_update} with data $\mySet{Q}^* = \mySet{Q}$ is likely to result in poor information error rates. Consequently, we opt to augment new data for training. In particular, our goal is to device an augmentation scheme $\psi:\mySet{Q} \mapsto \mySet{Q}^*$ such that, after training with $\mySet{Q}^*$, we result in parameters $\Weights$ that minimize  \eqref{eqn:ErrorRate}. 

% The above problem formulation considers a single channel realization. In practice, digital receivers often operate in block-fading channel conditions. In such cases,  each block of $B$ symbols undergoes a different channel, i.e., the statistical relationship between the channel outputs at the $j$th block $\{\myVec{y}_{i,j}\}_{i=1}^{\Blklen}$ and the  symbols $\{\myVec{s}_{i,j}\}_{i=1}^{\Blklen}$ varies with $j$. While each block requires a different receiver mapping $\Weights_j$, the data augmentation scheme $\psi$ can possibly fine tune itself between different realizations. For such settings, we are interested in data augmentation schemes that are {\em adaptive}, and are capable of leveraging past channel realizations to improve their ability to synthesize useful training data $\mySet{Q}^*$ from the current  pilots.
 

==> sections_v2/abstract.tex <==
\begin{abstract} 
\TomerFill{Deep neural networks (DNNs) allow digital receivers to learn to operate in complex environments. To do so, DNNs should  preferably be trained using large labeled data sets with a similar statistical relationship as the one under which they are to infer. For DNN-aided receivers, obtaining labeled data  conventionally involves pilot signalling at the cost of reduced spectral efficiency, typically resulting in access to limited data sets.
In this paper, we study how one can enrich a small set of labeled data into a larger data set for training deep receivers without transmitting more pilots. Motivated by the widespread use of data augmentation techniques for enriching visual and text data, we propose a dedicated augmentation scheme for exploiting the characteristics of digital communication data.  We identify the key considerations in data augmentations  for deep receivers as the need for domain orientation, class (constellation) diversity, and low complexity. Our method models each symbols class as Gaussian, using the available data to estimate its moments, while possibly leveraging data corresponding to related statistical models, e.g., past channel realizations, to improve the estimate.
The estimated clusters are used to enrich the data set by generating new samples used for training the DNN. The superiority of our approach is numerically evaluated for training a deep receiver on a linear and non-linear synthetic channels, as well as a COST 2100 channel. We show that our augmentation allows DNN-aided receivers to achieve gain of up to 3dB in \acl{ber}, compared to regular non-augmented training.} Should replace later.
\end{abstract}

==> sections_v2/conclusion.tex <==
\section{Conclusion}
	\label{sec:conclusion}
	\vspace{-0.1cm}
In this paper, we have proposed ...

==> sections_v2/dynamic.tex <==
% TODO NIR CONTINUE FROM HERE

\section{Data Augmentations for Dynamic Channels}
\label{sec:data_augmentations_dynamic}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/adaptive augmentation.PNG}
    \caption{Time-varying channels may benefit from an adaptive augmentation scheme.}
    \label{fig:adaptive_augmentation_illustration}
\end{figure}

In practice, digital receivers often operate in block-fading channel conditions. In such cases,  each block of $B$ symbols undergoes a different channel, i.e., the statistical relationship between the channel outputs at the $j$th block $\{\myVec{y}_{i,j}\}_{i=1}^{\Blklen}$ and the  symbols $\{\myVec{s}_{i,j}\}_{i=1}^{\Blklen}$ varies with $j$. While each block requires a different receiver mapping $\Weights_j$, the data augmentation scheme $\psi$ can possibly fine tune itself between different realizations. For such settings, we are interested in data augmentation schemes that are {\em adaptive}, and are capable of leveraging past channel realizations to improve their ability to synthesize useful training data $\mySet{Q}^*$ from the current pilots, as illustrated in Fig.~\ref{fig:adaptive_augmentation_illustration}. Since in this section the proposed scheme is adaptive, the mapping $\psi$ depends not only on the available data $\mySet{Q}$, but also on the previously used augmentation, i.e., the mapping applied in the previous block for block fading settings, denoted $\psi_{\rm prev}$. 

In block-fading settings, we propose to adaptively smooth the estimated clusters parameters \eqref{eq:mean_calculation} and \eqref{eq:variance_calculation} via a window smoothing approach. This way, we combine data across multiple time frames, meanwhile reducing the estimation noise. The motivation stems from the fact that  adjacent blocks may have different number of samples per class in each block, which induces high-variance noise. To reduce the noise effects, we exploit the continuous operation of \ac{dnn}-aided receivers and incorporate  adaptive smoothing, updating the clustering via
\begin{equation} \label{eq:smoothed_mean_calculation}
    \myVec{\mu}_j(\mypoint) = \frac{\beta_1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_{i,j} \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \myVec{y}_{i,j} + (1-\beta_1) * \myVec{\mu}_{j-1}(\mypoint) ,
\end{equation}
and
\begin{equation} \label{eq:smoothed_variance_calculation}
    \!\!\myMat{\Sigma}_j(\mypoint) \!=\!\frac{\beta_2}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_{i,j} \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \!\!\!\!(\myVec{y}_{i,j}\! - \!\myVec{\mu}_j(\mypoint))(\myVec{y}_{i,j} \!-\! \myVec{\mu}_j(\mypoint))^T + (1-\beta_2) * \myMat{\Sigma}_{j-1}(\mypoint).
\end{equation}
Here,  $\beta_1,\beta_2 \in [0,1]$ are hyperparameters  balancing the contribution of $\psi_{\rm prev}$ on $\psi$. For $\beta_1=\beta_2=1$, $\psi$ is not adaptive and is determined solely by $\mySet{Q}$, while for $\beta_1=\beta_2 = 0$, we have $\psi \equiv \psi_{\rm prev}$. 

To conclude the dynamic channel augmentation scheme $\psi_{dynamic}$, we follow the same guidelines of Algorithm~\ref{alg:StaticAugmentationScheme}, while replacing only lines \ref{line:centers_calculation} and \ref{line:variance_calculation} with the calculations in equations \eqref{eq:smoothed_mean_calculation} and \eqref{eq:smoothed_variance_calculation}, respectively.

==> sections_v2/introduction.tex <==
\section{Introduction}
\vspace{-0.1cm} 
	
% Paragraph - deep learning for receivers
% An alternative data-driven approach is based on deep learning. 
The emergence of deep learning has notably impacted numerous applications in various disciplines. %, ranging from computer vision and natural language processing to speech refinement and biomedical signal processing. 
The ability of \acp{dnn} to learn to efficiently carry out complex tasks from data has spurred a growing interest in their usage for receiver design in digital communications \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, farsad2020data}. The integration of model-agnostic trainable \acp{dnn}  in the receiver processing facilitates operation in complex scenarios where either a channel model deficit or an efficient algorithm deficit exist \cite{oshea2017introduction}, and can thus greatly contribute to meeting the constantly growing requirements of wireless systems in terms of throughput, coverage, and robustness \cite{saad2019vision}. 

% Following the same path, researchers in digital communication started to implement \ac{ml} driven solutions in classic communication components, such as antennas \cite{shlezinger2020dynamic}, reconfigurable intelligent surfaces \cite{alexandropoulos2021hybrid} and receivers \cite{gunduz2019machine,simeone2018very,balatsoukas2019deep, oshea2017introduction}. While traditional receiver algorithms are channel-model-based, relying on mathematical modeling \cite{xia2020mimo} of the signal transmission, propagation, and reception, \ac{dnn}-based receivers may facilitate operation in complex scenarios where either a channel model deficit or an efficient algorithm deficit exist \cite{shlezinger2020dynamic,alexandropoulos2021hybrid}, or difficult to optimize for~\cite{farsad2018neural,shlezinger2018asymptotic}.

% Paragraph - inherent challenge due to small available data sets
While deep learning thrives in domains such as computer vision or natural language processing, many challenges still limit its widespread applicability in digital communications. One of these challenges arises from the fact that \acp{dnn} rely on  (typically labeled) data sets to learn their mappings, and are thus usually applied when the  function being learned is stationary for a long period of time, such that one can collect sufficient data for learning. For example, data sets for machine translation tasks, which are nowadays dominated by deep learning systems, are usually composed of a sentence in an origin language, and its respective translation in a destination language, which does not change in time. One can thus collect millions or billions of such pairs for training, obtaining a huge data set for the task at hand. 
%
In contrast, the operation of digital receivers is rarely stationary, as communication channels (and thus the distribution of the data) change considerably over time. Moreover, \acp{dnn} are  highly-parameterized models, and their training requires massive data sets. In  digital receivers, labeled data corresponding to the current channel is obtained from pilots, whose transmission degrades the spectral efficiency. Thus, deployed digital receivers are likely to possess small labeled data sets, hardly in the scale needed to train \acp{dnn}. %This paper addresses the problem of small labeled data sets via augmentations. 
Consequently, a core challenge associated with the usage of \ac{dnn}-aided receivers stems from the need to aggregate sufficient task-specific data, i.e., data corresponding to the instantaneous setting where the receiver is required to operate.

%Augmentations refer to techniques that enrich the data set with new synthetic samples, with the augmentations presented in this paper being tailored to the communication domain.

%\subsection{Related Work}
Various strategies have been proposed  to facilitate the application of \acp{dnn}-aided receivers with limited data sets. 
The first approach trains with data obtained from simulations and past measurements and uses the limited data corresponding to the instantaneous channel to estimate some missing parameters, e.g., a channel matrix. These parameters are then used by the network, either as an input \cite{honkala2021deeprx,zhao2021deep} or as part of some internal processing  \cite{he2020model,khani2020adaptive, samuel2019learning, goutay2021machine,pratik2020re}. This  involves imposing a relatively simple model on the channel, typically a linear Gaussian model, which limits their suitability in the presence of complex channel models.  

An alternative approach designs receivers with compact task-specific \acp{dnn} such that they can be trained with relatively small data sets, by integrating them into classic receiver processing via model-based deep learning techniques \cite{shlezinger2020model, shlezinger2022model}, see, e.g., \cite{shlezinger2020data,shlezinger2019deepSIC, shlezinger2019viterbinet,raviv2020data}.
These hybrid model-based/data-driven receivers build on existing communication models and incorporate deep learning into their design, rather than replace the known model altogether with a black-box receiver. The resulting receivers are agnostic to the  channel model and its parameters, imitating the operation of a detection algorithm with no channel knowledge. Although these \ac{dnn}-aided receivers are compact in terms of trainable parameters, the amount of data required in training is still likely to be larger than the amount corresponding to the instantaneous channel one can typically obtain in real-time.

A third approach aims to optimize the training algorithm itself, rather than the architecture, facilitating rapid convergence of the training procedure with limited data.  Optimizing the hyperparameters that govern the optimization process is intuitively seen as a method to share data from different time steps, increasing the effective labeled data sets.
This can be achieved by leveraging  data corresponding to past channel realizations in order to tune the optimization hyperparameters via Bayesian optimization techniques~\cite{wang2021jointly}; model-agnostic meta-learning  \cite{park2020learning,park2020meta,simeone2020learning}; and predictive meta-learning which learns transition patterns in time-varying channels \cite{raviv2022online}. 
%distilling domain knowledge into the training algorithm itself \cite{park2020learning,park2020meta,simeone2020learning,raviv2021meta,raviv2022online}, rather than the architecture, facilitating rapid convergence of the training procedure with limited data. Namely, \ac{maml} \cite{finn2017model} is employed to calculate an inductive bias that allows quick re-training and adaption to different test scenarios, unseen at training time. Optimizing the hyperparameters that govern the optimization process is intuitively seen as a method to share data from different time steps, increasing the effective labeled data sets. Specifically, the method presented in \cite{raviv2022online} is tailored to rapidly time-varying channels, where the channel changes significantly between the consecutive packets.

The aforementioned strategies focus on either the architecture or the training algorithm. A complementary approach to cope with limited data sets, which can be combined with any of the above techniques, is to generate more data at the receiver. Current techniques aim at assigning labels to channel outputs not associated with pilots by exploiting the presence of channel coding for self-supervision \cite{shlezinger2019viterbinet, shlezinger2020inference, shlezinger2019deepSIC,teng2020syndrome} or by using active learning techniques \cite{be2019active, finish2022symbol}. However, these approaches cannot synthesize more data than the block length (typically generating much less \cite{finish2022symbol}), and the resulting data set may be too small for training.

A common practice in the deep learning literature  is to synthesize data samples via {\em data augmentation}. Data augmentation is a set of techniques that enrich a trainable model with new unseen synthetic data, where each technique builds on partial knowledge of the data  characteristics~\cite{shorten2019survey,nalepa2019data,feng2021survey,park2019specaugment}, typically exploiting some underlying translation invariance.  For instance, in image classification~\cite{shorten2019survey,nalepa2019data}, one can use a labeled image to generate multiple different images with the same label by, e.g., rotating or clipping it. While data augmentation is a widely used deep learning technique, it is highly geared towards the common image and language data. This motivates the study of augmentation techniques for enriching data in digital communications, as means to facilitate the training of \ac{dnn}-aided receivers with limited data sets.

\subsection*{Main Contributions}

% highlight our differences from previous or related works
In this paper we propose a data augmentation framework for \ac{dnn}-aided receivers. Our proposed method introduces a set of data synthesis techniques which exploit expected structures of digital communication channel outputs to enrich a small labeled data set with many reliable samples. The resulting enriched data can then be used for training, so as to reduce the error rate obtained by the receiver. 
Our main contributions are summarized as follows: 
\begin{itemize}
    \item \textbf{Proposed framework:} We formulate a communication-directed data augmentations framework, which embodies the specific characteristics of the digital communication data used for training \ac{dnn}-aided receivers.
    \item \textbf{Communications tailored augmentations:} We propose several augmentations that exploit innate traits of digital constellations. We exploit both expected symmetries in channel outputs as well as identified communication-specific translation invariance properties to generate new synthetic samples for training. 
    \item \textbf{Extensive experimentation:} \TomerFill{We extensively evaluate the proposed training scheme for both \ac{siso} and \ac{mimo} systems, considering different channel profiles. We demonstrate consistent benefits by using our approach with various \ac{dnn}-aided receivers, which amounts to gains of up to 3B compared with non-augmented training.} Detail the gains of our scheme once we finish the numerical part.
\end{itemize}

 The rest of this paper is organized as follows:  Section~\ref{sec:system_model} details the system model, while Section~\ref{sec:data_augmentations_static} formulates the frameworks and presents the augmentation techniques for static channels, where a single small data set corresponding to a specific channel realization is to be synthetically enriched for training. Section~\ref{sec:data_augmentations_dynamic} extends the augmentations to dynamic communication setups, accounting for continuous variations in block fading channels. Finally, experimental results and concluding remarks are detailed in Section~\ref{sec:numerical_evaluations} and Section~\ref{sec:conclusion}, respectively.

Throughout the paper, we use boldface letters for vectors, e.g., ${\myVec{x}}$; $({\myVec{x}})_i$ denotes
the $i$th element of ${\myVec{x}}$. %We use upper-case letters for \acp{rv}, and lower-case letters for deterministic quantities. 
Calligraphic letters, such as $\mySet{X}$, are used for sets, 
and $\mySet{R}$ is the set of real numbers.



==> sections_v2/results.tex <==
\section{Numerical Evaluations}
\label{sec:numerical_evaluations}
\vspace{-0.1cm} 
In this section we numerically evaluate the proposed augmentation schemes $\psi_{static}$ and $\psi_{dynamic}$ in finite-memory \ac{siso} channels and in memoryless multi-user \ac{mimo} setups\footnote{The source code used in our experiments is available at \href{https://github.com/tomerraviv95/data-augmentations-for-receivers}{https://github.com/tomerraviv95/data-augmentations-for-receivers}}. 
We first describe the receivers used in our experimental study, detailing the architectures in Subsection~\ref{subsec:simulated_receivers}. Then, we describe the compared augmented training methods in Subsection~\ref{subsec:augmentation_methods}. After presenting the setup, we introduce the main simulation results for the static augmentation scheme $\psi_{static}$, evaluated on linear synthetic channels, in Subsection~\ref{subsec:static_simulation_results}, and for evaluating the dynamic augmentation scheme $\psi_{dynamic}$ in Subsection~\ref{subsec:dynamic_cost_simulation_results} and Subsection~\ref{subsec:dynamic_synthetic_simulation_results} on non-linear synthetic channels and channels obeying the COST 2100 model, respectively. Finally, we provide ablation study for the contribution of each augmentation, and explore the efficiency of our augmentation scheme for different number of transmitted pilots in Subsection~\ref{subsec:ablation_study} and Subsection~\ref{subsec:pilots_efficiency}, respectively.

%-----------------------------------
%	Evaluated Equalizers
%-----------------------------------
\vspace{-0.4cm}
\subsection{Evaluated Receivers}
\label{subsec:simulated_receivers}
The receiver algorithms used in our experimental study vary based on the considered settings:
%\vspace{-0.1cm}
\subsubsection{Finite-Memory \ac{siso} Channels}
We compare two  \ac{dnn}-based receivers for \ac{siso} settings:
\begin{itemize}
    \item The ViterbiNet equalizer, proposed in \cite{shlezinger2019viterbinet}, which is a \ac{dnn}-based Viterbi detector \cite{viterbi1967error} for finite-memory channels. The Viterbi equalizer (from which ViterbiNet originates) solves the maximum likelihood sequence detection problem
\begin{align}
\hat{\myVec{s}}_j^{\rm info}   
&= \mathop{\arg \min}_{\myVec{s}_{i,j} \in \mySet{S} }\left\{-\sum\limits_{i= \Blklen^{\rm pilot} + 1}^{\Blklen^{\rm tran}} \log \Pdf{\myVec{Y}_{i,j} | \myVec{S}_{i-\Mem+1,j},\ldots, \myVec{S}_{i,j}}\left( \myVec{y}_{i,j}  |  \mypoint_{i-\Mem+1,j},\ldots, \mypoint_{i,j}\right)\right\}.
\end{align}	
    ViterbiNet computes each log likelihood using a  \ac{dnn} that requires no  knowledge of the channel  distributions $ \Pdf{\myVec{Y}_{i,j} |  \myVec{S}_{i-\Mem+1,j},\ldots, \myVec{S}_{i,j}}$. This internal \ac{dnn} is implemented using three fully-connected layers of sizes $1\times 100$, $100\times 50$, and $50 \times M^\Mem$, with activation functions set to sigmoid (after first layer), ReLU (after second layer), and softmax output layer.
    %sigmoid and ReLU activations, respectively, and a softmax output layer. 
    \item A recurrent neural network  symbol detector, comprised of a sliding-window \ac{lstm} \cite{tandler2019recurrent} with two hidden layers of $64$ cells and a window size of $1$. The output of the \ac{lstm} enters a fully-connected linear layer of size $64 \times M^\Mem$. This detector acts as a black-box \ac{dnn} benchmark. 
\end{itemize}

\subsubsection{Memoryless \ac{mimo} Channels}
We evaluate two  \ac{dnn}-based \ac{mimo}  receivers:
\begin{itemize}
    \item We adopt the DeepSIC receiver proposed in \cite{shlezinger2019deepSIC} as a modular receiver architecture. DeepSIC is derived from iterative \ac{sic} \cite{choi2000iterative}, which is a \ac{mimo}  detection method combining multi-stage interference cancellation with soft decisions. DeepSIC operates in $Q$ iterations, refining an estimate of the conditional \acl{pmf} of $\myVec{S}_k$, denoted by $\hat{\myVec{p}}_{k}^{(q)}$ where $q$ is the iteration number. This estimate   is generated for every symbol $k \in \{1,2,\ldots, K\}$ by using the corresponding estimates of the interfering symbols $\{S_l\}_{l \neq k}$ obtained in the previous iteration $\{\hat{\myVec{p}}_{\tilde{k}}^{(q-1)}\}_{\tilde{k}\neq k}$. Iteratively repeating this procedure refines the conditional distribution estimates, allowing the detector to accurately recover each symbol from the output of the last iteration. The building blocks of DeepSIC are implemented using three fully-connected layers:  An $(N + K - 1) \times 60$ first layer, a $60 \times 30$ second layer, and a $30 \times M^K$ third layer, with a sigmoid and a ReLU intermediate activation functions, respectively. The number of iterations is set to $Q=5$.  
    \item A black-box \ac{dnn} baseline using three fully-connected layers of sizes $N \times 60$, $60\times 60$, and $60 \times M^K$, with ReLU activation functions in-between and softmax output layer.
\end{itemize}

All receivers are trained by the adam optimizer for $500$ epochs, with batch size of $64$ and learning rate of $1e^{-3}$ for ViterbiNet and DeepSIC, batch size of $16$ and learning rate of $1e^{-2}$ for the LSTM black-box and batch size of $128$ and learning rate of $1e^{-2}$ for the linear fully-connected black-box. The receivers are trained until convergence at each time step.

% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.31\textwidth}
%     \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_train_channel.png}
%     \caption{Synthetic training channel.}
%     \label{fig:synthetic_train_channel}
%     \end{subfigure} 
%     %
%     \begin{subfigure}[b]{0.31\textwidth}
%     \includegraphics[width=\textwidth,height=0.15\textheight]{fig/synth_test_channel.png}
%     \caption{Synthetic test channel.}
%     \label{fig:synthetic_test_channel}
%     \end{subfigure}
%     % 
%     \begin{subfigure}[b]{0.31\textwidth}
%     \includegraphics[width=\textwidth,height=0.15\textheight]{fig/cost_channel.png}
%     \caption{COST 2100 channel.}
%     \label{fig:COSTChannel} 
%     \end{subfigure}
%     \caption{Examples of time-varying channels: channel coefficients versus block index.}
%     \figSpace
%     \label{fig:channels} 
%  %   \vspace{-0.1cm}
% \end{figure*}

\subsection{Augmentation Methods}
\label{subsec:augmentation_methods}
We compare the next training methods, including our proposed augmented training and a few baselines:
\begin{itemize}
    \item {\em Regular training}: No augmentations are applied; each receiver is trained using the original pilots batch $\mySet{Q}$ only.
    \item {\em Combined Scheme}: Our proposed augmentation technique $\psi_{static}$, which includes the sequential application of the geometric, translation and constellation-conserving projections as specified in Algorithm~\ref{alg:StaticAugmentationScheme}. In the case of time varying channels, as in Subsection~\ref{subsec:dynamic_cost_simulation_results} and Subsection~\ref{subsec:dynamic_synthetic_simulation_results}, we refer to $\psi_{dynamic}$ with $\beta_1=\beta_2=0.3$. The augmentation factor is chosen as $\kappa=4$ for all experiments, resulting in $|\mySet{Q}^*| = 5 \cdot |\mySet{Q}|$.
    \item {\em Extended pilot training}: Transmitting $2.5 \times$ the regular number of pilots, and training on the extended batch without any augmentations.
    % \item {\em Partial knowledge (PK) augmentation}: A genie-aided scheme that knows the instantaneous channel taps, and uses it to estimate the noise realizations.
    % Then, it synthesizes $K$ words per class by generating a random symbols word, convolve it with the  taps and add the estimated noise.
    % \item {\em Full knowledge (FK) augmentation}: A genie-aided scheme that knows the instantaneous channel taps and the \ac{snr}, and synthesizes $K * 2^\Mem$ words at each step of training. This schemes serves as a lower-bound on the achievable \ac{ber}.
\end{itemize}

%-----------------------------------
%	Simulation Results
%-----------------------------------
\vspace{-0.4cm}
\subsection{Results on Static Linear Gaussian Channels}
\label{subsec:static_simulation_results}
\vspace{-0.1cm}
We begin by evaluating Algorithm~\ref{alg:StaticAugmentationScheme} on stationary synthetic linear channels with additive Gaussian noise, considering  a finite-memory \ac{siso} setting and a memoryless \ac{mimo} setup.
%
\subsubsection{\ac{siso} Finite-Memory Channels} 
We transmit $\Blklen^{\rm pilot}=200$ pilots followed by $\Blklen^{\rm info}=10,000$ data bits, for a total transmission of a single block with size $\Blklen^{\rm tran}=10,200$. This means that only a small number of pilots are available to estimate the concurrent channel. We consider a linear Gaussian channel, whose input-output relationship is given by
\begin{equation}
\label{eqn:GaussianSISO}
\myVec{y}_i = \sum_{l=0}^{\Mem-1} \myVec{h}_{l}\myVec{s}_{i-l} + \myVec{w}_{i},
\end{equation}
where $\myVec{h} = [1,0.606,0.367,0.223]^T$ are the real channel taps, and $\myVec{w}_{i}$ is \acl{awgn} with variance $\sigma^2$. The channel memory is $\Mem = 4$ with the taps sampled from a synthetic model representing oscillations of varying frequencies. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/static_linear_synthetic_siso_BER_vs_SNR.png}
    \caption{\ac{siso} - \ac{ber} vs. SNR.}
    \label{fig:static_linear_synthetic_siso_BER_vs_SNR}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/static_linear_synthetic_mimo_BER_vs_SNR.png}
    \caption{\ac{mimo} - \ac{ber} vs. SNR.}
    \label{fig:static_linear_synthetic_mimo_BER_vs_SNR}
    \end{subfigure}
    %
    \caption{Static synthetic linear Gaussian channel.}
    \label{fig:static_linear_synthetic_BER_vs_SNR} 
    \figSpace
\end{figure*}

In Fig.~\ref{fig:static_linear_synthetic_siso_BER_vs_SNR} we plot the average \ac{ber}, as in equation \eqref{eqn:ErrorRate}, in conjunction with the various augmentations, when the \ac{snr}, defined as $1/\sigma^2$, is set to values in the range of $9$ dB - $13$ dB. Each point is averaged over 100 trials, to reduce the Monte Carlo estimation noise. This figure shows that the combined augmentation approach significantly outperforms the regular training,  demonstrating gains of around 0.35dB in the model-based ViterbiNet, and up to 1.2dB in the black-box RNN case. Our augmentations are tailored to the detection task, being agnostic to the actual structure of the receiver. Different  gains are expected for different receivers, based on the domain knowledge already Incorporated in the receiver itself .



\subsubsection{Memoryless MIMO Channels} 
To further validate that these gains also hold for the \ac{mimo} setting, we use the same values as before for $\Blklen^{\rm pilot}$, $\Blklen^{\rm info}$ and $\Blklen^{\rm tran}$. 
The input-output relationship of a the memoryless Gaussian \ac{mimo} channel is given by
\begin{equation}
\label{eqn:GaussianMIMO}
\myVec{y} = \myMat{H}\myVec{s} + \myVec{W},
\end{equation}
where $\myMat{H}$ is a known deterministic $N\times K$ channel matrix, and $\myVec{W}$ consists of $N$ i.i.d Gaussian \acp{rv}.  
We set the number of users and antennas to $K=N=4$. The channel matrix $\myMat{H}$ models spatial exponential decay, and its entries are given by
$\left( \myMat{H}\right)_{n,k} = e^{-|n-k|}$, for each $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$.  The transmitted symbols are generated from a \ac{bpsk} constellation in a uniform i.i.d. manner, i.e., $\mathcal{S}=\{\pm 1\}^4$.

As one may observe in Fig.~\ref{fig:static_linear_synthetic_mimo_BER_vs_SNR}, the gains are smaller but consistent. Since DeepSIC only needs short pilot blocks to reliably estimate the networks' parameters under the simple synthetic linear Gaussian case, the addition of either augmentations or more pilots is negligible. One the other hand, for the black-box architecture which is more data-hungry, the augmentations yield gains of up to 0.3dB, reaching close to the extended pilots baseline, especially in the low-to-medium \ac{snr} regime.

\begin{figure*}
    \centering
    %     
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.18\textheight]{fig/cost_channel.png}
    \caption{COST 2100 channel.}
    \label{fig:cost_channel_taps_siso} 
    \end{subfigure}
    % 
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.18\textheight]{fig/synth_test_channel.png}
    \caption{Synthetic channel.}
    \label{fig:synthetic_channel_taps_siso}
    \end{subfigure}
    % 
    \caption{\TomerFill{Time-varying \ac{siso} channels examples: channel coefficients versus block index.} To update.}
    \figSpace
    \label{fig:channels} 
\end{figure*}

\vspace{-0.4cm}
\subsection{Results on Time-Varying Linear COST Channels}
\label{subsec:dynamic_cost_simulation_results}
\vspace{-0.1cm}
Next, we evaluate the proposed augmentation scheme in time-varying linear channels. We choose to employ the COST 2100 model for generating the time-varying taps. The COST 2100 geometry-based stochastic channel model \cite{liu2012cost} is a widely used model to represent indoor wireless communications scenarios.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/varying_linear_cost_siso_BER_vs_SNR.png}
    \caption{\ac{siso} - \ac{ber} vs. SNR.}
    \label{fig:varying_linear_cost_siso_BER_vs_SNR}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/varying_linear_cost_mimo_BER_vs_SNR.png}
    \caption{\ac{mimo} - \ac{ber} vs. SNR.}
    \label{fig:varying_linear_cost_mimo_BER_vs_SNR}
    \end{subfigure}
    %
    \caption{\TomerFill{Time-varying COST 2100 linear Gaussian channel.} To update.}
    \label{fig:varying_linear_cost_BER_vs_SNR} 
    \figSpace
\end{figure*}

\subsubsection{\ac{siso} Finite-Memory Channels} We employ a similar linear model as in \ref{eqn:GaussianSISO}, but incorporate a time varying characteristics: 
\begin{equation}
\label{eqn:GaussianSISOvarying}
\myVec{y}_{i,j} = \sum_{l=0}^{\Mem-1} \myVec{h}_{l,j}\myVec{s}_{i-l,j} + \myVec{w}_{i,j},
\end{equation}
where the taps realizations $\myVec{h}_j = [\myVec{h}_{0,j},\ldots,\myVec{h}_{\Mem-1,j}]^T$ are generated using an indoor hall $5$ GHz setting with single-antenna elements, and $\myVec{w}_{i,j}$ is yet an \acl{awgn} with variance $\sigma^2$. The resulting channel taps are displayed in Fig.~\ref{fig:cost_channel_taps_siso}. 

We transmit 100 blocks, and measure the average \ac{ber} over all blocks and bits. The same configuration for $\Blklen^{\rm pilot} = 200$, $\Blklen^{\rm info} = 10,000$ and $\Blklen^{\rm tran} = 10,200$ holds, as before. Fig.~\ref{fig:varying_linear_cost_siso_BER_vs_SNR} shows the average results over 5 such trials (500 transmitted block in total). One may observe that gains of up to 1dB are achieved by employing our scheme. We can see that black-box have also achieved gains by employing the domain knowledge injected by our scheme. 

\subsubsection{Memoryless \ac{mimo} Channels} Similarly to the \ac{siso} case, we simulate a time-varying linear \ac{mimo} channel from \eqref{eqn:GaussianMIMO} via
\begin{equation}
\label{eqn:GaussianMIMOvarying}
\myVec{y}_j = \myMat{H}_j\myVec{s}_j + \myVec{W}_j,
\end{equation}
where the subscript $j$ expresses the time dependence of each term. The instantaneous channel matrix $H$ was simulated by following the above \ac{siso} description, and creating $4 \times 4 = 16$ \ac{siso} COST 2100 channels; Each simulated channel corresponds to a single entry $\left( \myMat{H}\right)_{n,k}$ with $n \in \{1,\ldots, N\}$, $ k \in \{1,\ldots, K\}$. Moving to results, calculated after the transmission of 100 blocks for 5 trials, one may observe that the respective graph Fig.~\ref{fig:varying_linear_cost_mimo_BER_vs_SNR} shows an unusual gain of up to 2dB approximately, as the regular training is unable to compete with the proposed approach.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/varying_non_linear_synthetic_siso_BER_vs_SNR.png}
    \caption{\ac{siso} - \ac{ber} vs. SNR.}
    \label{fig:varying_non_linear_synthetic_siso_BER_vs_SNR}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.48\textwidth}
    \includegraphics[width=\textwidth,height=0.22\textheight]{fig/varying_non_linear_synthetic_mimo_BER_vs_SNR.png}
    \caption{\ac{mimo} - \ac{ber} vs. SNR.}
    \label{fig:varying_non_linear_synthetic_mimo_BER_vs_SNR}
    \end{subfigure}
    %
    \caption{\TomerFill{Time-varying synthetic non-linear Gaussian channel.} To update.}
    \label{fig:varying_non_linear_synthetic_BER_vs_SNR} 
    \figSpace
\end{figure*}

\vspace{-0.4cm}
\subsection{Results on Time-Varying Non-Linear Synthetic Channels}
\label{subsec:dynamic_synthetic_simulation_results}
\vspace{-0.1cm}
Next, we evaluate the proposed online enrichment scheme in non-linear channels, where one can greatly benefit from the model-agnostic nature of \ac{dnn}-based receivers, as classical algorithm usually assume a linear Gaussian channel; \ac{dnn}-based receivers require no such assumption apriori. 

\subsubsection{\ac{siso} Finite-Memory Channels} To check the robustness of our method in a non-linear case, we generate such a channel by applying a non-linear transformation to the synthetic channel in \eqref{eqn:GaussianSISO}. The resulting finite-memory \ac{siso} channel is given by
\begin{equation}
\label{eqn:Gaussian1}
\myVec{y}_{i,j} =\tanh{\Big(C \cdot \Big(\sum_{l=0}^{\Mem-1} \myVec{h}_{l,j}\myVec{s}_{i-l,j} + \myVec{w}_{i,j}\Big)\Big)}.
\end{equation}
This operation may represent, e.g., non-linearities induced by the receiver acquisition hardware. The hyperparameter $C$ stands for a power attenuation at the receiver, and chosen empirically as $C=\frac{1}{2}$. All other hyperparameters and settings are the same as those used in the previous subsection. The channel taps follow a fading profile as depicted in Fig.~\ref{fig:synthetic_channel_taps_siso}.  

Looking at the aggregated gains of the 100 blocks transmission, the simulation shows empirically that a consistent gain of around $0.75$dB over the \ac{snr}s with values of $9$dB - $13$dB is accomplished, as observed in Fig.~\ref{fig:varying_non_linear_synthetic_siso_BER_vs_SNR}. The results here are averaged over 5 trials.

\subsubsection{Memoryless \ac{mimo} Channels} Similarly to the \ac{siso} case, we simulate a non-linear \ac{mimo} channel from \eqref{eqn:GaussianMIMO} via
\begin{equation}
\label{eqn:Gaussian2}
\myVec{y}_j = \tanh{\Big(C \cdot\Big(\myMat{H}_j\myVec{s}_j + \myVec{W}_j\Big)\Big)},
\end{equation}
with $C=\frac{1}{2}$ and the remaining simulation settings are chosen as in Subsection~\ref{subsec:dynamic_cost_simulation_results}. The numerical results for this channel are illustrated in Fig.~\ref{fig:varying_non_linear_synthetic_mimo_BER_vs_SNR}, showing that the superiority of our approach is maintained in non-linear setups. The results are an average over 5 trials. In particular, we note that gains of up to 0.5dB in high SNRs are achieved compared with online training, while the gap from regular training is around 0.25dB. Here, our gain becomes apparent as the SNR increases.

\vspace{-0.4cm}
\subsection{Ablation Study}
\label{subsec:ablation_study}
\vspace{-0.1cm}

Here we present the results when starting from regular training up to our augmentation scheme, showing that each augmentation adds a little to the proposed approach.

\vspace{-0.4cm}
\subsection{Pilots Efficiency}
\label{subsec:pilots_efficiency}
\vspace{-0.1cm}

Here we show curves of BER versus pilots for a chosen SNR, that is our approach is efficient in terms of transmission, showing effective pilot gains of 1.5X times.

==> sections_v2/static.tex <==
\section{Data Augmentations for Static Channels}
	\label{sec:data_augmentations_static}
	\vspace{-0.1cm}
Here, we present the proposed data augmentation techniques, considering a static setting, where one has access to a small data set corresponding to a single channel realization where it should also infer.
In Subsection~\ref{subsec:main_pillars} we introduce the rationale for using augmentations, and discuss the main pillars for data augmentation techniques in light of the operation of \ac{dnn}-aided communication receivers. We follow up with the communication-oriented augmentations in  Subsection~\ref{subsec:augmentations_static}, and provide a discussion in  Subsection~\ref{subsec:discussion}.  

%-----------------------------------
%	Main Pillars
%-----------------------------------
\vspace{-0.4cm}
\subsection{Rationale}
\label{subsec:main_pillars}

Data augmentation is a widely spread practice in machine learning. % for enriching a data set and for encouraging a trainable model to learn some known property of the data. 
For example, in speech processing, data augmentation includes several domain-tailored transforms such as time warping and frequency masking \cite{park2019specaugment}, which use observed sequences to generate new sequences the system should learn to cope with. In general, the purpose of using augmentations is to enrich the data set by exploiting domain knowledge regarding the nature of the data. The enriched set is then used for training the model with samples that may be observed during inference but are not included in the train set.

In digital communications, one is often faced with scarce data scenarios corresponding to a given task, i.e., when one has access to short packets which reflect on the channel coefficients at a specific time. As such, augmentations for communication applications can aid in obtaining new data for training \ac{dnn}-aided receivers. However, existing data augmentation techniques are highly geared towards structures and invariances exhibited by data in conventional machine learning domains such as visual, language, and speech data, and thus cannot be directly implemented in digital communications. 

% TODO NIR CONTINUE FROM HERE - what we discuss here are requirements and not really properties


% Therefore, in order 
% Our communication-oriented approach is differentiated from standard augmentations as it satisfies the following properties:
In the following sections, we develop augmentation techniques for data used by digital receivers.  Our approach accounts for the following data augmentation considerations:
\begin{enumerate}[label={\em C\arabic*}]
    \item \textbf{Domain-oriented} - \label{itm:domain} Data augmentations are inherently domain-oriented \cite{nooraiepour2021hybrid}. In our case, we exploit the inherent structure of digital constellations to formulate class-preserving transformations. 
    \item \textbf{Diversity} - \label{itm:diversiy}  The number of classes grows quickly with the system parameters such as the constellation size and the number of users. As such, the number of samples per class should be kept above some minimal threshold to avoid class imbalances \cite{be2019active,finish2022symbol}.
    \item \textbf{Complexity} - \label{itm:complexity} As data augmentation is to be implemented by a digital receiver in real-time, we must keep the sample-complexity low and the computation lightweight. 
\end{enumerate}

\begin{figure*}  % spans both columns
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/constellation.pdf}
\caption{Constellation points and received pilots}
\label{fig:constellation}
\end{subfigure}
\hfill % maximize the horizontal distance between the graphs
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/geometric.pdf}
\caption{Geometric augmentation}
\label{fig:geomtric}
\end{subfigure}

\bigskip  % some extra vertical whitespace
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/translation.pdf}
\caption{Translation augmentation}
\label{fig:translation}
\end{subfigure}
\hfill % maximize the horizontal distance between the graphs
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\linewidth]{fig/rotation.pdf}
\caption{Constellation-conserving rotation}
\label{fig:rotation}
\end{subfigure}

\caption{Augmentations exemplified on QPSK constellation} % Overall figure caption
\end{figure*}

% This is achieved by clustering the data based on the constellation symbol, and by adapting this clustering between blocks in block-fading channels as a form of temporal smoothing \cite{cambe2020exploring}.
%-----------------------------------
%	Augmentations
%-----------------------------------
\vspace{-0.4cm}
\subsection{Augmentations}
\label{subsec:augmentations_static}
%to design augmentation mechanisms, one must first identify th properties in digital communications data which can be exploited to synthesize new data. 

% \textcolor{red}{before going into the actual techniques, we should start with how we designed it. Particularly, what kind of models guide us in our design? We need to begin with a description of the following flavour:\\
% We draw our inspiration from common wireless communication models, where: \\
% 1. The channel output is often corrupted by additive distortion, e.g., noise and interference, which does not depend on the transmitted symbols. Thus we can often write $\myVec{y} = g(\myVec{s}) + \myVec{d}$ where $\myVec{d}$ is the additive distortion term that is invariance of $\myVec{s}$, and $g(\cdot)$ is the channel mapping capturing, e.g., the propagation environment between the transmitter and the receiver. This observation is what motivates our geometric augmentation and our translation augmentation. \\
% 2. Many constellations are symmetric, and thus there exist a discrete set of linear transformations which are constellation preserving, i.e., for every positive integer $n$ these exists a set of $n\times n$ matrices $\{\myMat{P}_i\}$ such that if  $\myVec{s}\in\mySet{S}^n$, it holds that   $\myMat{P}_i\myVec{s}\in\mySet{S}^n$ for each $i$. However, the channel mapping $g(\cdot)$  is not invariant to any such constellation preserving translation, and thus to build upon this property for augmentation one must  identify translations that are likely to be preserved by $g(\cdot)$. \\
% After we have this description, we can describe the following augmentation based on these properties and in light of considerations \ref{itm:domain}-\ref{itm:complexity}}

Designing communication-specific augmentations requires one to identify label-invariant transformations that must account for the statistical model, being the underlying input-output relationship induced by the communication model in our case. In the following, we detail three different and complementary augmentations: (1) geometric augmentation; (2) translation augmentation; and (3) constellation-reserving rotation. Each of these methods  originates from some expected wireless-communication behaviour.

\subsubsection{Geometric Augmentation} 
Our first augmentation technique draws inspiration from the common model of wireless channels as being decomposable into a channel response and an additive noise term. In such cases, one can write
\begin{equation}
    \label{eqn:addNoiseChannel}
    \myVec{y}=g(\myVec{s})+\myVec{n},
\end{equation}
where $g$ is the channel input-to-output transformation, and $\myVec{n}$ is an additive distortion term which is independent of $\myVec{s}$, e.g., thermal noise and interference.  This representation indicates that channel outputs corresponding to the same input tend to form clusters, as illustrated in Fig.~\ref{fig:constellation}, where the intra-cluster distribution is invariant of the center, as the noise is independent of the  signal. 
This geometrical interpretation of the by-class clusters can be employed to generate additional class-specific data.

In particular, we propose to use the existing labeled data $\mySet{Q}$ to identify clusters in the observations space from which the received symbols are likely to originate. Our method is based on clustering the channel outputs in $\mySet{Q}$ and setting $\myVec{\mu}$  and $\myMat{\Sigma}$ to be the cluster-wise centers and covariances, respectively.  %We characterize each cluster using its estimated first and second order statistical moments, which are estimated from the available data.
%empirically to cluster all received patterns per class via a Gaussian distribution. Each class distribution is dictated by two parameters, cluster center and its variance, both learned from the available pilots data.
%
Using the identified clusters, we suggest to synthesize data corresponding to a constellation point $\mypoint$ from a conditional Gaussian distribution $\mathcal{N}(\myVec{\mu}(\mypoint),\,\myMat{\Sigma}(\mypoint))$. 

Therefore, in order to enrich a labeled data set $\mySet{Q}$ into $\mySet{Q}^*$, we use $\mySet{Q}$ to determine $\myVec{\mu}$  and $\myMat{\Sigma}$ for each $\mypoint$. To that aim, we define the index set corresponding to $\mypoint$ as 
\begin{equation}
    \label{eqn:IdxSet}
    \mySet{I}_{\mySet{Q}}(\mypoint) := \{i| \mypoint_i \in \mySet{Q}; \mypoint_i =  \mypoint \}.
\end{equation}
We can now  estimate the moments of the clusters as
 \begin{equation} \label{eq:mean_calculation}
    \myVec{\mu}(\mypoint) =\frac{1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \myVec{y}_{i},
\end{equation}
and similarly 
 \begin{equation} \label{eq:variance_calculation}
    \!\!\myMat{\Sigma}(\mypoint) \!=\!\frac{1}{|\mySet{I}_{\mySet{Q}}(\mypoint)|} \sum_{\myVec{y}_i \in \mySet{Q}: i \in  \mySet{I}_{\mySet{Q}}(\mypoint)} \!\!\!\!(\myVec{y}_{i}\! - \!\myVec{\mu}(\mypoint))(\myVec{y}_{i} \!-\! \myVec{\mu}(\mypoint))^T.
\end{equation}
To avoid empty sets $\mySet{I}(\mypoint)$, one can opt pilot sequences for which each class has at least a single representative. The augmentation is depicted in Fig.~\ref{fig:geomtric}.
 %
Once the clusters are set, they are used to draw synthetic samples $\myVec{y}^{\prime}$ for some corresponding label $\mypoint^{\prime}$. %The tuple $(\myVec{y}^{\prime},\mypoint^{\prime})$ is the input to the next augmentation. 
  
\subsubsection{Translation Augmentation} 
In the previous augmentation we exploited data from a single constellation point to enrich it with new samples. To share and exploit data from different clusters, we propose a translation augmentation. Here, we again build upon the additive distortion model in \eqref{eqn:addNoiseChannel}, but instead of generating new samples around a given cluster in a random fashion, we synthesize a new {\em realization} of the distortion. This distortion is a weighted average of two computed distortions.

%\textcolor{blue}{To formulate this notion, let us take a commonly used model that assumes a channel output that is corrupted by additive distortion, e.g., noise and interference, which does not depend on the transmitted symbols. Thus, we can write $\myVec{y} = g(\myVec{s}) + \myVec{d}$ with $\myVec{d}$ being the additive distortion term that is invariant of the class $\myVec{s}$, and with $g(\cdot)$ being the channel mapping that captures the propagation environment between the transmitter and receiver. As the additive term $\myVec{d}$ is class-invariant, estimation of its value for a first class, also approximately holds for a second class. This observation is what motivates our translation augmentation.}. To that end, we translate geometric-augmented data points between different clusters. 

%\textcolor{red}{can we describe this in a way which does not divide whether SISO or MIMO? can we just use the general formulations of $\myVec{y}$ and $\myVec{s}$?}

To formalize this idea, let $\myVec{\mu}(\mypoint)$ be the cluster center estimated in \eqref{eq:mean_calculation}. We now introduce the empirical difference vector $\mydiff$, which measures the disparity of the channel output and the computed cluster center, i.e.,
\begin{equation} \label{eq:difference_calculation}
    \mydiff =\myVec{y} - \myVec{\mu}(\mypoint)
\end{equation}
and compute this value for all labeled samples $\mydiffSet = \{\mydiff_i^{\rm pilot}|i \in \{1,2,\ldots, \Blklen ^{\rm pilot}\} \}$. Then, considering a labeled pair $(\myVec{y}_i,\mypoint_i)$, one can generate a new unseen distortion $\mydiff^{\prime}$ by weighting the distortion of the $i^{\rm th}$ sample with a randomly sampled one $\mysampleddiff \in \mydiffSet$:
%\myVec{\mu}(\mypoint)
\begin{equation} \label{eq:difference_weighting}
     \mydiff^{\prime} =  \alpha * \mydiff_i + (1-\alpha) * \mysampleddiff.
\end{equation}
Then, to obtain the augmented pair $(\myVec{y}^{\prime},\mypoint^{\prime})$, we sample $\alpha \sim U[0,1]$ and add the synthetic distortion $\mydiff^{\prime}$ to the corresponding center $\myVec{y}^{\prime} = \myVec{\mu}(\mypoint^{\prime}) + \mydiff^{\prime}$ as illustrated in Fig.~\ref{fig:translation}.

\subsubsection{Constellation-Conserving Projections} 
Many constellations are symmetric by design. This means that there exists a discrete set of linear projections $\{{\myCCP}\}$ which are \textit{constellation-conserving}. A matrix $\myMat{P}^{\rm cc}$, with size of $|\mySet{S}| \times |\mySet{S}|$, represents a constellation-conserving projection if for every $\myVec{s}\in\mySet{S}$, it is satisfied that $\myCCP\myVec{s}\in\mySet{S}$ as well. This property may be exploited to generate additional training data when it meets the following two requirements:
\begin{itemize}
    \item The distribution of the noise is invariant to the transformation, i.e., that $\myVec{d}^{\rm cc} = \myCCP\myVec{d}$ obeys (approximately) the same distribution as  $\myVec{d}$.
    \item The channel mapping $g(\cdot)$ in \eqref{eqn:addNoiseChannel} (approximately) satisfies $ \myCCP g(\myVec{s}) \approx  g(\myCCP \myVec{s})$.
\end{itemize}
When the above hold, one can use a labeled pair $(\myVec{y}, \myVec{s})$ to generate additional data $(\myVec{y}^\prime, \myVec{s}^\prime)$ by noting that
\begin{equation}
\myVec{y}^\prime =\myCCP\myVec{y} = \myCCP g(\myVec{s}) + \myCCP\myVec{d} \approx  g(\myCCP\myVec{s}) + \myVec{d}^{\rm cc} = g(\myVec{s}^\prime) + \myVec{d}^{\rm cc}, 
\end{equation}
which is approximately identically distributed as an output obtained from the channel input $\myVec{s}^\prime = \myCCP \myVec{s}$.

% by applying it to the simplified model $\myMat{P}_u\myVec{y} = \myMat{P}_u g(\myVec{s}) + \myMat{P}_u\myVec{d}$ with two main requirements. First, we demand the distortion to be transformation-agnostic $\myMat{P}_u\myVec{d} \approx \myVec{d}$. Second, we assume  Under these requirements, the tuple $(\myMat{P}_u \myVec{y},\myMat{P}_u \myVec{s})$ may be added to the augmented batch for training. 

% TODO NIR CONTINUE FROM HERE
To design constellation-preserving augmentations, we note that communication channel mappings are often commutative to scalar multiplication, i.e., $g(a \myVec{s}) = a g(\myVec{s})$ for scalar $a$. This holds for instance, when the channel is linear. Consequently, we focus on the discrete rotations transformations, for which $\myCCP = e^{j \pi \frac{\phi}{180}} \myMat{I}$. For example, under a  QPSK constellation ($M=4$), one can set $\phi = \frac{2\pi m}{4}$ for any $m \in \{0,1,2,3\}$ such that $\myCCP \myVec{s}$ is a valid constellation point. Furthermore, the distribution of noise signals is often rotation-invariant as is the case for, e.g., circularly-symmetric Gaussian $\myVec{d}$. Consequently, permutations of such case are likely to be constellation-preserving and satisfy the above requirements. 

The resulting proposed augmentation operates by randomly choosing $\myCCP$ out of the corresponding set $\{\myCCP\}$ and applying it to the pair samples: 
\begin{equation} \label{eq:constellation_conserving_rotation}
     \myVec{y}^{\prime} = \myCCP \myVec{y},\quad 
     \mypoint^{\prime} = \myCCP \mypoint.
\end{equation}
The augmented pair $(\myVec{y}^{\prime},\mypoint^{\prime})$ is added to the buffer $\mySet{Q}^*$. See an illustration of a synthetic example in Fig.~\ref{fig:rotation}.

\subsubsection{Combined Scheme} 
Each of the aforementioned methods allows to generate additional new data from an available labeled set comprised of channel outputs and their corresponding transmitted symbols. As these methods are complementary of each other, we combine them into an overall data augmentation method  by applying them subsequently.  

First, we initialize the buffer by $\mySet{Q}^*=\mySet{Q}$. To realize the diversity consideration \ref{itm:diversiy}, we augment each sample into $\kappa$ new samples. Then, we add all synthetic samples to the augmented training batch $\mySet{Q}^*$, resulting in a set of $(\kappa+1)* \cdot |\mySet{Q}|$ labeled samples to be used for training $\Weights$, as illustrated in Fig.~\ref{fig:transmission}. Note the each augmentation may be applied on its own, or in consecutive pairs. However, we provide empirical demonstration in Section~\ref{sec:numerical_evaluations} that augmented pairs that are the output of two different augmentations are usually independent of each other, causing the gain from each augmentation to sum up. The resulting combined augmentation policy $\psi_{static}:\mySet{Q} \mapsto \mySet{Q}^*$ for static channels is formulated in full as Algorithm~\ref{alg:StaticAugmentationScheme}.

\begin{figure}
  \begin{algorithm}[H]
    \caption{Static Channel Augmentation Scheme $\psi_{static}$}
    \label{alg:StaticAugmentationScheme}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwFor{RepTimes}{repeat}{times}{end}
    \SetKwProg{AugmentationScheme}{Augmentation Scheme}{}{}
    \Input{data set $\mySet{Q}$; \newline augmentation factor $\kappa$} %  \newline 
 %   \Output{augmented batch $\mySet{Q}^*$}
    \AugmentationScheme{$(\mySet{Q},K)$}{
        $\myVec{\mu}(\mypoint) \gets$ calculate by  \eqref{eq:mean_calculation}, $\forall \mypoint \in \mySet{S}$\;\label{line:centers_calculation}
        
        $\myMat{\Sigma}(\mypoint) \gets$ calculate by  \eqref{eq:variance_calculation}, $\forall \mypoint \in \mySet{S}$\;\label{line:variance_calculation}
        
        $\mydiffSet \gets$ calculate by  \eqref{eq:difference_calculation}, $\forall \myVec{s}_i^{\rm pilot} \in \mySet{Q}$\;\label{line:diff_set_calculation}


    Initialize $\mySet{Q}^* = \mySet{Q}$\;
    \RepTimes{$\kappa$}{
    \For{$\mypoint_i$ in $\mySet{Q}$}{%
                
                \nonl\texttt{Geometric Augmentation}\;

                sample $\myVec{y}^{\prime}$ from $\mathcal{N}(\myVec{\mu}(\mypoint_i),\,\myMat{\Sigma}(\mypoint_i))$;\label{line:sample_from_distribution}
                
                \nonl\texttt{Translation Augmentation}\;
                
                $\myVec{d}^{\prime} \gets$ calculate from $\myVec{y}^{\prime}$ by  \eqref{eq:difference_weighting}\;\label{line:difference_weighting}
                 $\myVec{y}^{\prime\prime} \gets \myVec{\mu}(\mypoint_i) + \mydiff^{\prime}$\;\label{line:difference_addition}
                
                \nonl\texttt{Constellation-Conserving Rotation}\;
                
                choose a random $\myCCP$\;
             $\myVec{y}^{\prime\prime\prime},\myVec{s}^{\prime\prime\prime} \gets$ rotation by \eqref{eq:constellation_conserving_rotation}\;
              \nonl\texttt{Buffer update}\;
                add $(\myVec{y}^{\prime\prime\prime},\mypoint^{\prime\prime\prime})$ to buffer $\mySet{Q}^*$; \label{line:add_to_buffer}
                
                }}
        \KwRet{$\mySet{Q}^*$}
  }
  \end{algorithm}
\end{figure}

%-----------------------------------
%	Discussion
%-----------------------------------
\vspace{-0.4cm}
\subsection{Discussion}
\label{subsec:discussion}

Algorithm~\ref{alg:StaticAugmentationScheme} integrates data augmentation into digital receiver processing, synthesizing channel outputs data from the input pilots. This data allows the receiver to train without relying on lengthy pilot transmissions, achieving accurate training with short pilots as empirically demonstrated in Section~\ref{sec:numerical_evaluations} and increasing the effective transmitted pilots size. The suggested  policy differs from augmentations in other domains, e.g., vision, being specifically tailored to communications. This domain knowledge includes the geometrical interpretation of the channel outputs which follows from the typical arrangements of digital constellations; the expected balanced symbol diversity as communication symbols are typically uniformly distributed; and the symmetry of common constellations. in the following section we show how one can also incorporate knowledge regarding the continuous operation of digital receivers, which allows to benefit from the presence of past channels and data, while also restricting to framework to light computations. Contrary to other domains, where augmentations often rely on complex policies, e.g., using generative networks \cite{almahairi2018augmented} or reinforcement learning \cite{laskin2020reinforcement}, we keep our mechanism light. The operations required for our scheme include: sampling from a Gaussian distribution, adding and subtracting vectors and lastly multiplying by a phase. These operations allow our mechanism to be carried out in real time.

Algorithm~\ref{alg:StaticAugmentationScheme} can be combined with other approaches for training deep receivers with scarce data. These approaches include the model-based methods \cite{shlezinger2020model}, as well as self-supervision methods \cite{finish2022symbol,shlezinger2019viterbinet}, which assign decision-directed labels to  channel outputs and uses them for training. While self-supervision cannot generate more samples than the block length, Algorithm~\ref{alg:StaticAugmentationScheme} can synthesize any number of samples, and is thus suitable for coping with short block lengths. 


==> sections_v2/system_model.tex <==
\section{System Model}
\label{sec:system_model}
\vspace{-0.1cm}

In the section, present the system model. To that aim, we first describe the communication model in Subsection~\ref{subsec:communication_model}, and the we discuss the receiver processing and the considered problem formulation of data augmentation for \ac{dnn}-aided receivers in Subsection~\ref{subsec:Receiver}. 

%-----------------------------------
%	Communication Model
%-----------------------------------
\vspace{-0.2cm}
\subsection{Communication Model}
\label{subsec:communication_model}
\vspace{-0.1cm} 
We consider a generic digital communication system in discrete-time. 
Let $\myVec{s}_i\in\mySet{S}$ be a symbol transmitted from constellation $\mySet{S}$ (with its size denoted $|\mySet{S}|$) at the $i$th time instance, $i \in \{1,2,\ldots, \Blklen ^{\rm tran}\} = \Blkset$. The transmitted symbols block $\mys ^{\rm tran}:= \{\myVec{s}_i\}_{i\in \Blkset}$ with length $B^{\rm tran}$, is divided into $\Blklen^{\rm pilot}$ pilots that are known to the receiver,  denoted $\myVec{s}^{\rm pilot}$, and  $\Blklen^{\rm info} = \Blklen^{\rm tran}-\Blklen^{\rm pilot}$ information symbols $\myVec{s}^{\rm info}$ that are unknown. The channel output at time instance $i$ is denoted by $\myVec{y}_i$, which takes some value in the set $\mySet{Y}$, and the received block is $\myVec{y}^{\rm rec}:= \{\myVec{y}_i\}_{i\in \Blkset}$. It can be separated by the receiver, similarly as the channel input, into its pilot and information parts denoted $\myVec{y}^{\rm pilot}$ and $\myVec{y}^{\rm info}$, respectively. We assume that the channel, i.e., the mapping from $\myVec{s}$ into $\myVec{y}$, is constant within a block of $\Blklen^{\rm tran}$ channel uses, which thus corresponds to the coherence duration of the channel. 

{\bf Channel Models:} 
While the above channel model is generic, we focus mostly on the common setting of communication over casual finite-memory channels. 
We note two important cases of this channel model, which are also the ones considered in our experimental study:
\begin{enumerate}
    \item \emph{\ac{siso} Finite-Memory Channels}: In multipath \ac{siso} channel, the channel output $\myVec{y}_{i}$ is given by a stochastic function of the last $\Mem > 0$ transmitted values, where $\Mem$ is the memory length. The constellation size is $|\mySet{S}|=M^L$ where $M$ is the alphabet size. We set $\myVec{s}_i \equiv \myVec{0}$ for $i<0$, i.e., we assume a guard interval of at least $\Mem-1$ time instances prior to the beginning of the block.
    \item \emph{Flat \ac{mimo} Channels}: Another channel of interest is the memoryless \ac{mimo} channel, where $|\mySet{S}|=M^K$ and $|\mySet{Y}|=\mySet{R}^N$ with $K>1$ and $N>1$. The variable $K$ denotes the number of single-antenna transmitters (users), and for $K>1$ the setting represents a multiple access channel. The variable $N$ represents the number of receive antennas. %We denote $\mystate_i \equiv \myVec{s}_i$ in this case, for ease of notation.
\end{enumerate}
%For both channels, one can replace $\myVec{s}_i$ with $\mystate_i$ in \eqref{eq:meta_1}, \eqref{eqn:ErrorRate} and in $\mySet{Q}= \{(\myVec{y}_i^{\rm pilot},\mystate_i^{\rm pilot}) \}$.

%-----------------------------------
%	Receiver
%-----------------------------------
\vspace{-0.2cm}
\subsection{Receiver Operation and Problem Formulation}
\label{subsec:Receiver}
\vspace{-0.1cm} 
The receiver processing is aided by a  \ac{dnn} which relies on labeled data to learn its mapping. In particular, the receiver recovers the information symbols from $\myVec{y}^{\rm info}$ using a \ac{dnn}-aided detection mapping, which yields the estimate $\hat{\myVec{s}}(\myVec{y}^{\rm info}; \Weights)$, where  $\Weights$  are the  parameters of the \ac{dnn}.
The parameters $\Weights$ are obtained by training, using the available labeled data representing the underlying channel which is denoted by $\mySet{Q}^*$.
The training module follows a (stochastic) gradient-based optimization with empirical loss measure $\mySet{L}_{\mySet{Q}^*}$, e.g., iterations of the form
 \begin{align}
\label{eq:local_update} % \label{eq:meta_1}
\Weights^{(t+1)} = \Weights^{(t)} - \eta \hat{\nabla}_{\Weights}\mySet{L}_{\mySet{Q}^*}(\Weights^{(t)}),
 \end{align}
 where $\eta > 0$ is the learning rate and $\hat{\nabla}_{\Weights}\mySet{L}$ is a stochastic approximation of the gradient of the empirical loss with respect to the trainable parameters. Since symbol detection is a classification task, we focus on $\mySet{L}_{\mySet{Q}^*}$ being the empirical cross-entropy loss, such that \eqref{eq:local_update} approximates the solution to
 \begin{align}
\label{eq:meta_1}
  \mathop{\arg \min}_{\Weights} \Big\{ \mySet{L}_{\mySet{Q}^*}(\Weights) = -\sum_{(\myVec{y}_i, \myVec{s}_i) \in\mySet{Q}^* }\log \hat{P}_{\Weights}\left(\myVec{s}_{i}|\myVec{y}_{i} \right)\Big\},
\end{align}
with $\hat{P}_{\Weights}(\cdot|\cdot)$ representing the soft (probabilistic) estimates produced by the receiver with \ac{dnn} parameters $\Weights$.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/communication scheme.PNG}
    \caption{System model illustration.}
    \label{fig:transmission}
\end{figure}

While the \ac{dnn}-aided receiver trains with a labeled data set for which the transmitted symbols are known, its performance is measured in its ability to recover the information data. Consequently, the considered performance measure for evaluating the parameters $\Weights$ trained via \eqref{eq:local_update} is the \ac{ber} over the information block 
\begin{equation}
\label{eqn:ErrorRate}
	e(\Weights) = \frac{1}{\Blklen^{\rm info}}\sum_{i= \Blklen^{\rm pilot} + 1}^{\Blklen^{\rm tran}} \Pr\left( \hat{\myVec{s}}_i(\myVec{y}^{\rm info};\Weights) \neq  \myVec{s}_i^{\rm info} \right). 
\end{equation} 
An illustration of the system is depicted in Fig.~\ref{fig:transmission}. 

{\bf Problem Formulation:} 
Note that the labeled data set corresponding to the current channel to which the receiver has access is  $\mySet{Q}= \{(\myVec{y}_i^{\rm pilot},\myVec{s}_i^{\rm pilot})|i \in \{1,2,\ldots, \Blklen ^{\rm pilot}\} \}$, i.e., the known pilots and their respective received values.  When the number of samples $B^{\rm pilot}$ is relatively small, training via \eqref{eq:local_update} with data $\mySet{Q}^* = \mySet{Q}$ is likely to result in poor information error rates. Consequently, we opt to augment new data for training. In particular, our goal is to device an augmentation scheme $\psi:\mySet{Q} \mapsto \mySet{Q}^*$ such that, after training with $\mySet{Q}^*$, we result in parameters $\Weights$ that minimize  \eqref{eqn:ErrorRate}. 

% The above problem formulation considers a single channel realization. In practice, digital receivers often operate in block-fading channel conditions. In such cases,  each block of $B$ symbols undergoes a different channel, i.e., the statistical relationship between the channel outputs at the $j$th block $\{\myVec{y}_{i,j}\}_{i=1}^{\Blklen}$ and the  symbols $\{\myVec{s}_{i,j}\}_{i=1}^{\Blklen}$ varies with $j$. While each block requires a different receiver mapping $\Weights_j$, the data augmentation scheme $\psi$ can possibly fine tune itself between different realizations. For such settings, we are interested in data augmentation schemes that are {\em adaptive}, and are capable of leveraging past channel realizations to improve their ability to synthesize useful training data $\mySet{Q}^*$ from the current  pilots.
 
